Mammo-FM: Breast-specific foundational model for Integrated Mammographic Diagnosis, Prognosis, and Reporting

Breast cancer is one of the leading causes of death among women worldwide. We introduce Mammo-FM, the first foundation model specifically for mammography, pretrained on the largest and most diverse dataset to date - 140,677 patients (821,326 mammograms) across four U.S. institutions. Mammo-FM provides a unified foundation for core clinical tasks in breast imaging, including cancer diagnosis, pathology localization, structured report generation, and cancer risk prognosis within a single framework. Its alignment between images and text enables both visual and textual interpretability, improving transparency and clinical auditability, which are essential for real-world adoption. We rigorously evaluate Mammo-FM across diagnosis, prognosis, and report-generation tasks in in- and out-of-distribution datasets. Despite operating on native-resolution mammograms and using only one-third of the parameters of state-of-the-art generalist FMs, Mammo-FM consistently outperforms them across multiple public and private benchmarks. These results highlight the efficiency and value of domain-specific foundation models designed around the full spectrum of tasks within a clinical domain and emphasize the importance of rigorous, domain-aligned evaluation.

==> sections/abstract_v1.tex <==
% what is the problem:

% why people care about the problem
% what makes it hard problem
% GAP
% Solution
% justify the impact



% Problem and importance:In 2022, breast cancer accounted for 2.3 million new cases and 666,000 deaths globally, making it the most diagnosed cancer worldwide  - breast cancer is popular cancer. Detecting it early necessary. Lots of woman goes for screening  - radiologists are over worked for diagnosis. Also, the radiologist spent lot of time taking notes - they are overworked and fatigued.

%  AI FM models can be helpful here. One potential strategy is to construct robust vision–language models for mammography using generalist models, such as MedGemma or cxr models 
% Problems in them: low resolution, First, generalist models
% often operate on downsampled images or low-resolution patches, a strategy that fails to capture sub-
% tle, diagnostically critical features such as microcalcifications and architectural distortions unique
% to mammography. Also, not focusing on mammo is another problem. it results poor zero-shot and data efficiency performance. Rich features can be not be exatractd from exisiting interpretable risk predictors AsymMIRAI as they use shallow vis encoders resnet18. And report generation as well bcz the image encoder is bad and the lang model also not follow the reporting strucuture of mammo bcz they are not finetuned.

% he problems. Existing models in generalist FM can help in diagnosis and report gen. Existing models like asym mirai can help inn interpretable risk prediction but they have problems and den discuss the problems in First 2nd etc. 1 problem is low res. 2nd problem is modality specific training 3rd problem is the vis encoder used in gen AI models like medgemma 4 th problem is the generated reports from generalist models dont follow mammo specific style.

% Our contribution: 1st vis-lang model on mammograms mammo-clip, trained with multiinstitution large scale (195,976 studies) real screening mammo and reports data. handle large images. it captures rich feartures, useful for risk prediction and report generation. Report generations model mammo-GRG finetuned on 298,285 mammography QA pair derived from real reports. 

% Rigourous evaluation: classificatioon of mammo findings and cancer both ID and OOD setting. Detection of mammo findings. Risk pred in ID and OOD. Report generations using GREEN metric - compare generated vs predicted report, findings identification from reports. Outperforms all the tasks w.r.t baselines medgemma, medSigCLIP (classification, vis encoder of medgemma), DINOv3, CXR-CLIP etc


Breast cancer represents a significant global health challenge, with 2.3 million new cases and 666,000 deaths recorded in 2022. Early detection through screening mammography is essential, but expanding screening programs increases the workload on radiologists, leading to diagnostic fatigue and a substantial documentation burden. 
Current artificial intelligence models offer potential solutions for mammography: generalist foundation models, such as MedGemma, aim to assist with diagnosis and automated reporting, while prognosis models like AsymMIRAI provide interpretable risk prediction. However, all of them suffer from critical limitations. First, generalist models operate on downsampled, low-resolution images, failing to capture diagnostically critical features \eg microcalcifications. Second, without pretraining on high-resolution, modality-specific images, these models cannot learn the necessary visual priors, resulting in poor performance in zero-shot classification and data inefficiency tasks. Third, the vision encoders in AsymMIRAI, which include the shallow architecture, are insufficient for extracting the rich features required for robust risk prediction. Finally, reports generated by generalist models lack clinical fidelity, as they are not fine-tuned to the specific structure, terminology, and style of mammography reporting. 
This paper introduces Mammo-CLIP, the first vision-language foundation model, pre-trained on a large-scale, multi-institutional dataset of 195,976 real-world screening studies and reports. Mammo-CLIP extracts rich visual features from high-resolution mammograms, essential for downstream clinical applications. Leveraging these representations, we demonstrate two key downstream applications: (1) interpretable risk prediction using bilateral asymmetry, and (2) multi-view report generation through Mammo-GRG, a model instruction-tuned on 298,285 question-answer pairs derived from real reports and grounded by zero-shot visual findings. Rigorous evaluation across both in-distribution and out-of-distribution settings demonstrates that Mammo-CLIP, the interpretable risk predictor, and Mammo-GRG outperform all the generalist baselines (MedGemma, MedSigLIP, DINOv3, and CXR-CLIP) for classification, localization, risk prediction, and report generation tasks. Overall, these results highlight the importance of domain-specific pretraining in achieving clinically reliable and interpretable mammography AI systems. 

==> sections/abstract_v2.tex <==
Breast cancer represents a significant global health challenge, with 2.3 million new cases and 666,000 deaths recorded in 2022. Early detection through screening mammography is essential, but expanding screening programs increases the workload on radiologists, leading to diagnostic fatigue and a substantial documentation burden. 
Current artificial intelligence models offer potential solutions for mammography: generalist foundation models, such as MedGemma, aim to assist with diagnosis and automated reporting, while prognosis models like AsymMIRAI provide interpretable risk prediction. However, all of them suffer from critical limitations. First, generalist models operate on downsampled, low-resolution images, failing to capture diagnostically critical features \eg microcalcifications. Second, without pretraining on high-resolution, modality-specific images, these models cannot learn the necessary visual priors, resulting in poor performance in zero-shot classification and data inefficiency tasks. Third, the vision encoders in AsymMIRAI, which include the shallow architecture, are insufficient for extracting the rich features required for robust risk prediction. Finally, reports generated by generalist models lack clinical fidelity, as they are not fine-tuned to the specific structure, terminology, and style of mammography reporting. 
This paper introduces Mammo-CLIP, the first vision-language foundation model, pre-trained on a large-scale, multi-institutional dataset comprising screening mammograms and reports from 195,976 patients. Mammo-CLIP extracts rich visual features from high-resolution mammograms, essential for downstream clinical applications. Leveraging these representations, we demonstrate two key downstream applications: (1) interpretable risk prediction using bilateral asymmetry, and (2) multi-view report generation through Mammo-GRG, a model instruction-tuned on 298,285 question-answer pairs derived from real reports and grounded by zero-shot visual findings. Rigorous evaluation across both in-distribution and out-of-distribution settings demonstrates that Mammo-CLIP, the interpretable risk predictor, and Mammo-GRG outperform all the generalist baselines (MedGemma, MedSigLIP, DINOv3, and CXR-CLIP) for classification, localization, risk prediction, and report generation tasks. This work establishes a clear path toward developing trustworthy, domain-specific AI that can alleviate radiologist burden, enhance diagnostic precision, and support a more scalable future for breast cancer screening.

==> sections/abstract_v3.tex <==
Breast cancer is one of the leading causes of death among women worldwide. We develop the first foundation model (FM) specifically designed for mammography, pretrained on the largest and most diverse dataset to date -- 140,677 patients (821,326 screening mammograms) -- across four institutions in the US. The model serves as a single foundation for key clinical tasks in breast cancer screening: diagnosing suspicious findings, estimating future cancer risk, and generating radiology reports consistent with clinical standards. 
Our design follows four principles. First, data efficiency: the model captures high-resolution mammographic features \eg masses, tissue density \etc, enabling accurate zero-shot classification and lightweight fine-tuning. Second, diagnostic and prognostic efficiency: it delivers high predictive performance for both cancer detection and forward risk estimation, supporting patient prioritization and triage. Third, multimodal interpretability: its vision–language alignment enables downstream risk prediction models to achieve image- and text-based interpretability. Fourth, structured report generation: the model produces clinically coherent radiology reports from screening mammograms
Our model satisfies all four criteria, establishing a scalable foundation for breast cancer AI. Our mammography-specific FM (only 8B parameters in total with a 30M-parameter vision encoder) outperforms the current generalist FMs \eg MedGemma (27B parameters in total with 400M-parameter vision encoder), on multiple public benchmarks across diagnosis, prognosis, and report generation at a fraction of the computational cost.
This paper demonstrates that true generalization in clinical imaging is driven by organ-specific pretraining, not by sheer parameter scale or heterogeneous pretraining data.

% This work demonstrates that organ-specific pretraining -- not scale in paramteres and training data -- drives true generalization in clinical imaging

% , showing that organ-specific specialization -- not scale-- drives true generalization in clinical imaging.
% This work demonstrates that tailored foundation models can surpass generalist architectures when aligned with the needs of a specific clinical domain.

% One punch missing. 1st report generator and 1st text interpretable prognosis
% Size punch
% organ specific domain generalization
% Moreover, our FM also provides, for the first time, multimodal (both image- and text-based) interpretability for existing risk predictors, a capability not achievable with their conventional, non-language-aligned encoders. 

==> sections/abstract_v4.tex <==
Breast cancer is one of the leading causes of death among women worldwide. We introduce the first foundation model (FM) specifically for mammography, pretrained on the largest and most diverse dataset to date -- 140,677 patients (821,326 mammograms) -- across four US institutions.
Our design follows four principles: 1) capturing high-resolution mammographic features, enabling accurate zero-shot classification and lightweight fine-tuning; 2) delivering accurate cancer detection and forward risk estimation, supporting patient prioritization and triage; 3) enabling image- and text-based interpretability to the downstream risk predictor due to vision–language alignment of the FM; 4) generating clinically coherent radiology reports from mammograms.
For the first time in breast cancer AI, our model (8B total parameters; 30M-parameter vision encoder) satisfies all four criteria and outperforms the generalist FMs \eg MedGemma (27B total parameters; 400M-parameter vision encoder), on multiple public benchmarks at a fraction of the pretraining cost.
Our results demonstrates that organ-specific pretraining, not scale, drives clinical generalization in medical imaging.


% The model serves as a single foundation for key clinical tasks in breast cancer screening: diagnosing suspicious findings, estimating future cancer risk, and generating radiology reports consistent with clinical standards.








==> sections/diagnosis_v1.tex <==
% * why do we need this experiment
% * experimental setup
% * baselines
% * metric
% * dataset
% * important result

% what do we offer - the 1st sent

We evaluate Mammo-CLIP across in-distribution (ID) and out-of-distribution (OOD) settings. The ID evaluation leverages the public EMBED dataset to classify mass, suspicious calcification, architectural distortion, and cancer. For OOD evaluation, we utilize the public VinDr (to classify mass, density, calcification, and cancer) and RSNA (to classify cancer) datasets, as they were excluded from pretraining (Tab.~\ref{tab:dataset_eval_characteristics}). We evaluate Mammo-CLIP under four complementary settings. First, for zero-shot classification, we compute image-text similarity using aligned encoders without task-specific training (Fig.~\ref{fig:diagnosis}a, Methods). Refer to Fig.~\ref{fig:app_image_label_augment} for the prompts used in zero-shot evaluations. Second, for linear probing, we train a linear classifier on the frozen vision encoder using training subsets from 10\% to 100\% (Fig.~\ref{fig:diagnosis}c). Third, for full fine-tuning, we optimize the entire model (both the vision encoder and classifier) for cancer classification on RSNA and VinDr. Fourth, for detection, we integrate the vision encoder into a fine-tuned RetinaNet architecture (Fig.~\ref{fig:diagnosis}e, Methods). We benchmark Mammo-CLIP against multiple baselines, including a UPMC-only variant, generalist FMs (\eg MedSigLIP the vision encoder of MedGemma), chest-X-ray models (\eg CXR-CLIP-RN50), and self-supervised models (\eg DINOv3). We report classification and detection performance using AUROC and mAP, respectively.


\begin{figure}[p]
    \centering
    \includegraphics[width=0.81\textwidth]{figures/diagnosis.pdf}
    \vspace{-0.8em}
    \caption{\textbf{Evaluation of Mammo-CLIP representations for diagnosing mammographic findings.} \textbf{a.} Schematic overview of zero-shot classification, where aligned image and text encoders predict the presence of mammographic findings (\eg mass, calcification) by measuring image–text embedding similarity, without task-specific training. \textbf{b.} Zero-shot evaluation of breast cancer and finding classification performance on in-distribution (ID; EMBED) and out-of-distribution (OOD; VinDr, RSNA) datasets. \textbf{c.} Illustration of the linear probing setup, in which only a classification head is trained atop the frozen vision encoder to assess representation quality. \textbf{d.} Schematic of the full fine-tuning configuration, where the entire model is optimized end-to-end for downstream diagnostic tasks. \textbf{e.} Data efficiency analysis across ID and OOD datasets, showing progressive improvement in classification performance with increasing fractions of training data. \textbf{f.} Pathology localization performance using a RetinaNet detection framework with a Mammo-CLIP vision encoder as backbone. \textbf{g.} Pathology localization performance detecting mass and calcification from VinDr dataset. \textbf{h-i}, Quantitative results for OOD and ID classification under full fine-tuning (top panels) and linear probing (bottom panels), reported as AUROC. Across all tasks and datasets, Mammo-CLIP (multi-institution) shows higher diagnostic accuracy, superior generalization, and data efficiency compared with single-institution, generalist, and self-supervised baselines -- highlighting the importance of domain-specific, multi-institutional pre-training for clinically robust mammographic representation learning. In all the evaluations, we denote suspicious calcification as calcification for brevity.}  
    \label{fig:diagnosis}
\end{figure}

Mammo-CLIP (multi-institution) outperforms all baselines across ID and OOD  classification across all four evaluation settings. In zero-shot classification, it achieves 13–38\% higher AUROC than MedSigLIP across tasks ($P<0.001$ for all; Fig.~\ref{fig:diagnosis}b) without any task-specific fine-tuning. Specifically, for zero-shot cancer classification, it achieves AUROCs of 0.75 (95\% CI: 0.72–0.76) on RSNA and 0.83 (95\% CI: 0.80–0.84) on VinDr, yielding $\sim25$\% and $\sim22$\% relative improvements over MedSigLIP. The multi-institutional pretraining is critical; compared with its UPMC-only variant, the multi-institutional model demonstrates 13–15\% higher AUROC on OOD zero-shot cancer classification for both the datasets. In the linear-probe setting, Mammo-CLIP (multi-institution) shows strong OOD generalization across the different tasks (Fig.~\ref{fig:diagnosis}h bottom and Fig.~\ref{fig:diagnosis}i right). Specifically, for OOD calcification classification on VinDr, Mammo-CLIP (multi-institution) achieves an AUROC of 0.94 (95\% CI: 0.90–0.97), representing a 27\% and 11\% improvement over MedSigLIP (AUROC 0.74, 95\% CI: 0.72-0.78; $P = 0.003$) and the single-institution UPMC variant (AUROC 0.88, 95\% CI: 0.85–0.90; $P = 0.003$), respectively. A similar trend follows for other tasks across EMBED, VinDr and RSNA datasets. This superior performance demonstrates the multi-institutional model's robust generalization to unseen populations, such as the Vietnamese cohort in VinDr. 

Full fine-tuning further reinforces the multi-institutional model's superior performance (Fig.~\ref{fig:diagnosis}h top and Fig.~\ref{fig:diagnosis}i left panel). For OOD cancer classification on VinDr, Mammo-CLIP (multi-institution) achieves an AUROC of 0.93 (95\% CI: 0.92–0.94). This denotes an 18\% improvement over MedSigLIP (AUROC 0.79, 95\% CI: 0.78–0.81; $P = 0.003$) and a 34\% improvement over the UPMC variant (AUROC 0.69, 95\% CI: 0.68–0.70; $P = 0.003$). Mammo-CLIP's performance on cancer classification is notable, as it is pretrained on screening mammograms, where reports do not explicitly mention cancer or malignancy. 
Refer to Fig.~\ref{fig:app_density} for the similar results of breast density classification.  Fig.~\ref{fig:diagnosis}g reports the results of pathology localization tasks. For mass detection, the fine-tuned multi-institution Mammo-CLIP achieves a mAP of 0.58 (95\% CI: 0.55–0.62), a 12\% ($P = 0.005$) improvement over the UPMC variant (mAP = 0.52; 95\% CI: 0.50–0.55). We restrict comparisons to CNN-based models, as the localization pipeline leverages a RetinaNet backbone. 

These results establish Mammo-CLIP (multi-institution) as a comprehensive diagnostic foundation model. It consistently outperforms generalist and single-institution baselines
across ID and OOD public benchmarks across all four evaluation settings. These findings show that large-scale, domain-specific, multi-institutional pretraining is essential for robust, transferable clinical vision-language models for mammography.d0

==> sections/discussion_v1.tex <==

% not punchy? positive of generalist and criticise with spealist.

% \textbf{Discussion in pointers like ML/CV conference.}
% The results highlight three key limitations of existing generalist vision–language models when applied to 2D mammography, and demonstrate how Mammo-CLIP addresses each through domain-specialized pretraining and architectural design.

% \textbf{1. Generalist pretraining fails to capture domain-specific features.}
% Models such as MedGemma, CXR-CLIP, MedCLIP, and GLoRIA are pretrained on large-scale datasets but are not specialized for mammography. MedGemma uses heterogeneous medical image–text pairs, while CXR-CLIP and MedCLIP rely on chest X-ray datasets (e.g., MIMIC-CXR, CheXpert). These models exhibit poor zero-shot performance on mammography tasks, suggesting limited transferability of general-purpose medical pretraining.

% Mammo-CLIP is pretrained exclusively on high-resolution 2D mammograms, allowing it to learn clinically relevant structures such as mass boundaries, microcalcifications, and architectural distortion patterns. This results in superior performance on both in-distribution (EMBED) and out-of-distribution (VinDr, RSNA) benchmarks.

% \textbf{2. Low input resolution limits detection of fine-grained features.}
% Most generalist models operate at restricted input resolutions (e.g., GLoRIA: 256×256; MedCLIP, CXR-CLIP: 224×224; MedGemma: 896×896), which are suboptimal for mammography, where critical features are often subtle and small.

% Mammo-CLIP processes full-resolution inputs at 1520×912, preserving spatial fidelity required for accurate classification of fine-grained imaging features. This contributes to improved performance, particularly in tasks involving calcifications and architectural distortion.

% \textbf{3. Limited institutional diversity reduces generalization.}
% Single-institution training and conventional contrastive objectives may not support robust performance across varying clinical sources. For example, Mammo-CLIP (UPMC) and CLIP-ENB5(UPMC) are trained on identical data, but show lower performance than Mammo-CLIP trained on multi-institutional data.

% Mammo-CLIP employs a multi-view contrastive loss and leverages data from UPMC, BU, and Mayo Clinic, enabling it to learn view-consistent and distributionally robust representations. This leads to consistent improvements across all evaluation settings.



% Our results highlights the advantages of domain-specialized pretraining on high-resolution 2D mammography data for building robust vision–language models. Generalist models \eg MedGemma and   CXR-based models \eg CXR-CLIP, MedCLIP, and GLoRIA, though trained on large-scale and diverse medical corpora, consistently underperform in both in-distribution and out-of-distribution mammography tasks. While generalist vision–language models offer broad applicability and data efficiency, they exhibit key limitations for breast imaging. First, mammography is a high-resolution, modality-specific domain where learning fine-grained visual features is essential for capturing breast anatomy and identifying subtle abnormalities. Generalist models often rely on patch-based encoding at low resolution (\eg 224×224 in CXR-CLIP and MedCLIP, 256×256 in GLoRIA). Such low resolution constrains their ability to capture diagnostic features such as microcalcifications or architectural distortions. In contrast, Mammo-CLIP operates at 1520×912 resolution and is trained exclusively on mammograms, enabling it to preserve spatial detail critical for accurate representation.
% %  (Mention about zero-shot, finetuning and linear probe)
% Second, although generalist models are designed to learn transferable visual–textual representations, they do not transfer effectively to dense, high-stakes modalities like mammography. Mammo-CLIP, pretrained on a domain-specific corpus of high-resolution images and associated radiology reports, demonstrates superior generalization across multiple external datasets without requiring downstream fine-tuning. The results indicate that aligning images and reports within a single imaging modality learns better robust and task-relevant features than generalist pretraining across heterogeneous domains. Moreover, while generalist models may offer clinical flexibility, reliability and diagnostic precision are critical in breast cancer screening. n modality-constrained settings, performance cannot be traded off for model flexibility.

% Mammo-CLIP (UPMC) outperforms CLIP-ENB5 (UPMC) across all evaluation tasks, despite both models being trained on the same single-institution dataset. Such performance gain illustrates the importance of Mammo-CLIP’s multi-view supervision loss, which learns shared feature representations across CC and mediolateral oblique MLO views of the same breast. In contrast, CLIP-ENB5 employs a standard image–text contrastive loss and processes each view independently, without leveraging anatomical correspondence between CC and MLO views of the same breast. Pretraining Mammo-CLIP on multi-institutional data yields further improvements, emphasizing the importance of dataset scale and distributional diversity for developing generalizable foundation models. Together, these findings emphasize the role of both architecture-level design and training data diversity in improving robustness and transferability for breast imaging tasks.



Our results highlight the advantages of domain-specialized pretraining on high-resolution 2D mammography data for building robust vision–language models. Generalist models—such as MedGemma—and chest X-ray–based models—such as CXR-CLIP, MedCLIP, and GLoRIA—though trained on large-scale and diverse medical corpora, consistently underperform in both in-distribution and out-of-distribution mammography tasks. While generalist vision–language models offer broad applicability and data efficiency, they exhibit key limitations for breast imaging.

First, mammography is a high-resolution, modality-specific domain where learning fine-grained visual features is essential for representing breast anatomy and identifying subtle abnormalities. Generalist models often rely on patch-based encoding at low resolution (\eg 896$\times$896 in MedGemma, 224$\times$224 in CXR-CLIP and MedCLIP, 256$\times$224256 in GLoRIA). Such low resolution constrains their ability to capture diagnostic features \eg calcifications or architectural distortions. In contrast, Mammo-CLIP processes images at 1,520$\times$912 resolution and is pretrained exclusively on mammograms, enabling it to preserve spatial detail critical for breast imaging tasks.

Second, although generalist models aim to learn transferable visual–textual representations, they fail to generalize effectively to dense, high-stakes modalities like mammography. Mammo-CLIP, pretrained on a domain-specific corpus of high-resolution images and radiology reports, achieves strong zero-shot performance across external datasets—without any downstream training—highlighting the value of aligned image–text supervision within a single modality. Linear probing with a frozen encoder shows that Mammo-CLIP yields more discriminative features than generalist or CXR–based models, indicating that mammography-specific pretraining enables effective feature transfer under limited supervision. Full fine-tuning further amplifies the performance of Mammo-CLIP, reflecting the strength of initialization provided by mammography-specific pretraining. These trends are consistent across both in-distribution (EMBED) and out-of-distribution (VinDr) datasets, illustrating the robustness of the learned features to domain shift.

Importantly, Mammo-CLIP generalizes to cancer classification tasks, even though its pretraining corpus—based on 2D screening exams—did not contain explicit cancer annotations. Across both EMBED (in-distribution) and RSNA (out-of-distribution), Mammo-CLIP consistently outperforms generalist and CXR-based models, establishing its adaptability to clinically critical targets not represented in pretraining. Further evaluation with a RetinaNet-based model shows that the Mammo-CLIP encoder accurately localizes masses and calcifications, indicating that its breast-specific representations are applicable to tasks beyond classification.

Mammo-CLIP (UPMC) outperforms CLIP-ENB5 (UPMC) across all evaluation tasks, despite both models being trained on the same single-institution dataset. Such performance gain illustrates the importance of Mammo-CLIP’s multi-view supervision loss, which learns shared feature representations across CC and mediolateral oblique MLO views of the same breast. In contrast, CLIP-ENB5 employs a standard image–text contrastive loss and processes each view independently, without leveraging anatomical correspondence between CC and MLO views of the same breast. Pretraining Mammo-CLIP on multi-institutional data yields further improvements, emphasizing the importance of dataset scale and distributional diversity for developing generalizable foundation models. Together, these findings emphasize the role of both architecture-level design and training data diversity in improving robustness and transferability for breast imaging tasks.

\subsection*{Discussion.}
% not punchy? positive of generalist and criticise with spealist.

% Our results highlight the importance of domain-specialized pretraining on high-resolution 2D mammography data for building robust vision–language models. Despite being trained on large-scale datasets, generalist models \eg MedGemma and CXR-based models \eg CXR-CLIP, MedCLIP, and GLoRIA, consistently underperform across both in-distribution and out-of-distribution tasks. MedGemma is trained on diverse medical image–text data, and CXR-CLIP and MedCLIP incorporate large-scale chest X-ray datasets (e.g., MIMIC-CXR, CheXpert) with paired image–text and image–label supervision. Nevertheless, these models are less effective in representing mammographic features, likely due to their lack of specialization in 2D mammography.
% In contrast, Mammo-CLIP leverages pretraining exclusively on high-resolution mammograms (1520×912), enabling it to capture task-relevant fine-grained structures such as calcifications and distortions. This resolution notably exceeds that of MedGemma (896×896), GLoRIA (256×256), and CXR-CLIP and MedCLIP (both 224×224), allowing Mammo-CLIP to model spatial detail critical for breast imaging tasks. Furthermore, Mammo-CLIP pretrained on multi-institutional data outperforms its UPMC-only counterpart, emphasizing the importance of dataset scale and distributional diversity for generalization. Compared to CLIP-ENB5, which uses the same UPMC data but standard contrastive loss, Mammo-CLIP benefits from a multi-view contrastive learning objective tailored to mammography’s multi-view acquisition protocol.

% \textbf{Discussion in pointers like ML/CV conference.}
% The results highlight three key limitations of existing generalist vision–language models when applied to 2D mammography, and demonstrate how Mammo-CLIP addresses each through domain-specialized pretraining and architectural design.

% \textbf{1. Generalist pretraining fails to capture domain-specific features.}
% Models such as MedGemma, CXR-CLIP, MedCLIP, and GLoRIA are pretrained on large-scale datasets but are not specialized for mammography. MedGemma uses heterogeneous medical image–text pairs, while CXR-CLIP and MedCLIP rely on chest X-ray datasets (e.g., MIMIC-CXR, CheXpert). These models exhibit poor zero-shot performance on mammography tasks, suggesting limited transferability of general-purpose medical pretraining.

% Mammo-CLIP is pretrained exclusively on high-resolution 2D mammograms, allowing it to learn clinically relevant structures such as mass boundaries, microcalcifications, and architectural distortion patterns. This results in superior performance on both in-distribution (EMBED) and out-of-distribution (VinDr, RSNA) benchmarks.

% \textbf{2. Low input resolution limits detection of fine-grained features.}
% Most generalist models operate at restricted input resolutions (e.g., GLoRIA: 256×256; MedCLIP, CXR-CLIP: 224×224; MedGemma: 896×896), which are suboptimal for mammography, where critical features are often subtle and small.

% Mammo-CLIP processes full-resolution inputs at 1520×912, preserving spatial fidelity required for accurate classification of fine-grained imaging features. This contributes to improved performance, particularly in tasks involving calcifications and architectural distortion.

% \textbf{3. Limited institutional diversity reduces generalization.}
% Single-institution training and conventional contrastive objectives may not support robust performance across varying clinical sources. For example, Mammo-CLIP (UPMC) and CLIP-ENB5(UPMC) are trained on identical data, but show lower performance than Mammo-CLIP trained on multi-institutional data.

% Mammo-CLIP employs a multi-view contrastive loss and leverages data from UPMC, BU, and Mayo Clinic, enabling it to learn view-consistent and distributionally robust representations. This leads to consistent improvements across all evaluation settings.



% Our results highlights the advantages of domain-specialized pretraining on high-resolution 2D mammography data for building robust vision–language models. Generalist models \eg MedGemma and   CXR-based models \eg CXR-CLIP, MedCLIP, and GLoRIA, though trained on large-scale and diverse medical corpora, consistently underperform in both in-distribution and out-of-distribution mammography tasks. While generalist vision–language models offer broad applicability and data efficiency, they exhibit key limitations for breast imaging. First, mammography is a high-resolution, modality-specific domain where learning fine-grained visual features is essential for capturing breast anatomy and identifying subtle abnormalities. Generalist models often rely on patch-based encoding at low resolution (\eg 224×224 in CXR-CLIP and MedCLIP, 256×256 in GLoRIA). Such low resolution constrains their ability to capture diagnostic features such as microcalcifications or architectural distortions. In contrast, Mammo-CLIP operates at 1520×912 resolution and is trained exclusively on mammograms, enabling it to preserve spatial detail critical for accurate representation.
% %  (Mention about zero-shot, finetuning and linear probe)
% Second, although generalist models are designed to learn transferable visual–textual representations, they do not transfer effectively to dense, high-stakes modalities like mammography. Mammo-CLIP, pretrained on a domain-specific corpus of high-resolution images and associated radiology reports, demonstrates superior generalization across multiple external datasets without requiring downstream fine-tuning. The results indicate that aligning images and reports within a single imaging modality learns better robust and task-relevant features than generalist pretraining across heterogeneous domains. Moreover, while generalist models may offer clinical flexibility, reliability and diagnostic precision are critical in breast cancer screening. n modality-constrained settings, performance cannot be traded off for model flexibility.

% Mammo-CLIP (UPMC) outperforms CLIP-ENB5 (UPMC) across all evaluation tasks, despite both models being trained on the same single-institution dataset. Such performance gain illustrates the importance of Mammo-CLIP’s multi-view supervision loss, which learns shared feature representations across CC and mediolateral oblique MLO views of the same breast. In contrast, CLIP-ENB5 employs a standard image–text contrastive loss and processes each view independently, without leveraging anatomical correspondence between CC and MLO views of the same breast. Pretraining Mammo-CLIP on multi-institutional data yields further improvements, emphasizing the importance of dataset scale and distributional diversity for developing generalizable foundation models. Together, these findings emphasize the role of both architecture-level design and training data diversity in improving robustness and transferability for breast imaging tasks.



Our results highlight the advantages of domain-specialized pretraining on high-resolution 2D mammography data for building robust vision–language models. Generalist models—such as MedGemma—and chest X-ray–based models—such as CXR-CLIP, MedCLIP, and GLoRIA—though trained on large-scale and diverse medical corpora, consistently underperform in both in-distribution and out-of-distribution mammography tasks. While generalist vision–language models offer broad applicability and data efficiency, they exhibit key limitations for breast imaging.

First, mammography is a high-resolution, modality-specific domain where learning fine-grained visual features is essential for representing breast anatomy and identifying subtle abnormalities. Generalist models often rely on patch-based encoding at low resolution (\eg 896$\times$896 in MedGemma, 224$\times$224 in CXR-CLIP and MedCLIP, 256$\times$224256 in GLoRIA). Such low resolution constrains their ability to capture diagnostic features \eg calcifications or architectural distortions. In contrast, Mammo-CLIP processes images at 1,520$\times$912 resolution and is pretrained exclusively on mammograms, enabling it to preserve spatial detail critical for breast imaging tasks.

Second, although generalist models aim to learn transferable visual–textual representations, they fail to generalize effectively to dense, high-stakes modalities like mammography. Mammo-CLIP, pretrained on a domain-specific corpus of high-resolution images and radiology reports, achieves strong zero-shot performance across external datasets—without any downstream training—highlighting the value of aligned image–text supervision within a single modality. Linear probing with a frozen encoder shows that Mammo-CLIP yields more discriminative features than generalist or CXR–based models, indicating that mammography-specific pretraining enables effective feature transfer under limited supervision. Full fine-tuning further amplifies the performance of Mammo-CLIP, reflecting the strength of initialization provided by mammography-specific pretraining. These trends are consistent across both in-distribution (EMBED) and out-of-distribution (VinDr) datasets, illustrating the robustness of the learned features to domain shift.

Importantly, Mammo-CLIP generalizes to cancer classification tasks, even though its pretraining corpus—based on 2D screening exams—did not contain explicit cancer annotations. Across both EMBED (in-distribution) and RSNA (out-of-distribution), Mammo-CLIP consistently outperforms generalist and CXR-based models, establishing its adaptability to clinically critical targets not represented in pretraining. Further evaluation with a RetinaNet-based model shows that the Mammo-CLIP encoder accurately localizes masses and calcifications, indicating that its breast-specific representations are applicable to tasks beyond classification.

Mammo-CLIP (UPMC) outperforms CLIP-ENB5 (UPMC) across all evaluation tasks, despite both models being trained on the same single-institution dataset. Such performance gain illustrates the importance of Mammo-CLIP’s multi-view supervision loss, which learns shared feature representations across CC and mediolateral oblique MLO views of the same breast. In contrast, CLIP-ENB5 employs a standard image–text contrastive loss and processes each view independently, without leveraging anatomical correspondence between CC and MLO views of the same breast. Pretraining Mammo-CLIP on multi-institutional data yields further improvements, emphasizing the importance of dataset scale and distributional diversity for developing generalizable foundation models. Together, these findings emphasize the role of both architecture-level design and training data diversity in improving robustness and transferability for breast imaging tasks.



==> sections/discussion_v2.tex <==
% Overall narrative must be critiquing generalist models and  motivate for specialized domain models


% <para1>Motivating AI in Breast cancer assessment Reiterate the impact of breast cancer: most important form of cancer and pronosis early can help in survival. Also, radilogist are overworked in note taking. AI can help here. 
% (There must be a good transition sentence for the next paragraph to maintain the flow or coherence of motivating FM development)

% <para2>Problems in exisiting FMs: Traditional methods of FM is focused on building generalist models , pretrained on a wide array of datasets and modalities, intending to do well in wide array of downstream tasks. Mammo-CLIP is not doing in that way. It is only trained on screen mammo making it spealised model only to solve problems in mammography. It is trained on a large corpora of screening mammo and radiologist reports.
% This paper shows it outpeforms the generalist models (mention the model) in all the tasks (mention the tasks)
% Our results highlight the advantages of domain-specialized pretraining on high-resolution 2D mammography data for building robust vision–language models. Generalist models—such as MedGemma, image models like DINOv3, —and chest X-ray–based models—such as CXR-CLIP —though trained on large-scale and diverse medical corpora, consistently underperform in both in-distribution and out-of-distribution mammography tasks.
% While generalist vision–language models offer broad applicability and data efficiency, they exhibit key limitations for breast imaging.

% <para3>
% Why mammo-clip is so good? Mammo-clip is great in 
% Why mammo-clip 
% First, mammography is a high-resolution, modality-specific domain where learning fine-grained visual features is essential for representing breast anatomy and identifying subtle abnormalities. Generalist models often rely on patch-based encoding at low resolution (\eg 896$\times$896 in MedGemma, 224$\times$224 in CXR-CLIP also mention for DINOv3). Such low resolution constrains their ability to capture diagnostic features \eg calcifications or architectural distortions. In contrast, Mammo-CLIP processes images at 1,520$\times$912 resolution and is pretrained exclusively on mammograms, enabling it to preserve spatial detail critical for breast imaging tasks.
% Second, although generalist models aim to learn transferable visual–textual representations, they fail to generalize effectively to dense, high-stakes modalities like mammography. Mammo-CLIP, pretrained on a domain-specific corpus of high-resolution images and radiology reports, achieves strong zero-shot performance across external datasets—without any downstream training—highlighting the value of aligned image–text supervision within a single modality. Linear probing with a frozen encoder shows that Mammo-CLIP yields more discriminative features than generalist or CXR–based models, indicating that mammography-specific pretraining enables effective feature transfer under limited supervision. Full fine-tuning further amplifies the performance of Mammo-CLIP, reflecting the strength of initialization provided by mammography-specific pretraining. These trends are consistent across both in-distribution (EMBED) and out-of-distribution (VinDr) datasets, illustrating the robustness of the learned features to domain shift.
% Importantly, Mammo-CLIP generalizes to cancer classification tasks, even though its pretraining corpus—based on 2D screening exams—did not contain explicit cancer annotations. Across both EMBED (in-distribution) and RSNA (out-of-distribution), Mammo-CLIP consistently outperforms generalist and CXR-based models, establishing its adaptability to clinically critical targets not represented in pretraining. Further evaluation with a RetinaNet-based model shows that the Mammo-CLIP encoder accurately localizes masses and calcifications, indicating that its breast-specific representations are applicable to tasks beyond classification.
%  Pretraining Mammo-CLIP on multi-institutional data yields further improvements, emphasizing the importance of dataset scale and distributional diversity for developing generalizable foundation models. Together, these findings emphasize the role of both architecture-level design and training data diversity in improving robustness and transferability for breast imaging tasks.
% Getting these features from vis encoder is important for report generation Mammo-GRG. As, there we have to freeze the vision encoder. 
% Also, the rich alignment helps in prognosis.
% why the report generator Mammo-GRG is doing so good? Unlike existing generalist models, it uses mammo-clip spealized image representations. Plus unlike other models, it uses positional emnbeddings and other stuff to handle 4 views of mammograms at the same time. ALso the LLM for report generation is finetuned with  Question-answers derived from real world mammography reports. Finally the final reports are generated after going through a grounding stage which has mammo-clip image encoder,

% <para4> Impact:
% Good diagnosis - reduce the load from radiologist.
% good representation - helps / is essentail in deriving good prognostic model and good report generator
% interpretable prognosis than baseline
% Excellent report generator (Mammo-GRG) - reduce burden of radiologist from notetaking
%  Specialized models like mammo-clip excels in all aspect than generalist models

% <para4>: Limitations:
% Mammo-CLIP Pretraining datasets may have biases
% MIRAI as KD. So, biases encoded in MIRAI may come to the risk predictor.
% Third, it is worthnoting that zero-shot classification using prompts may be unstable because variations in the prompt could alter the results
% Report generator can depend on the choice of LLMs

% <para5>: oneline summary and concluding remark: This is an example In summary, our study demonstrates that AI transparency annd trustworthiness at scale are feasible in a way that was previously impossible: through image–text models tailored to the medical domain of interest.

% Main message. Domain specifc model outperform generalist models

Breast cancer remains the most prevalent cancer worldwide and the leading cause of cancer-related mortality in women. Early risk assessment plays a decisive role in reducing mortality, yet radiologists face increasing demands due to rising screening volumes and excessive burdens of documentation. Manual note-taking and report composition impose repetitive overhead, diverting time from tasks that more directly support interpretation and clinical reasoning. Artificial intelligence offers a path to augment radiologists’ capacity, automate low-level reporting, and improve diagnostic precision. This motivation inspires the development of mammography-specific foundation models that integrate visual understanding and clinical decision-making.

Current development of foundation models in medical AI emphasizes generalist strategies (\eg MedGemma): pretraining on diverse datasets across multiple modalities with the goal of universal applicability. Although this paradigm supports broad transferability, it fails in domains that demand fine-grained, modality-specific understanding like mammography. Our work diverges from this generalist trajectory. Our vision language model, Mammo-CLIP, is pretrained exclusively on the largest and most diverse multi-institutional corpus of screening mammograms and radiology reports to date, resulting in a foundation model specialized for the breast imaging domain. Across zero-shot classification, linear probing, full fine-tuning, and pathology localization, Mammo-CLIP consistently outperforms generalist models \eg MedSigLIP, DINOv3, and CXR-CLIP in both in-distribution and out-of-distribution settings. Notably, Mammo-CLIP achieves these results with an EfficientNet-based vision encoder of only 30 million parameters, whereas MedSigLIP employs a 400-million-parameter generalist encoder. This contrast highlights that scaling parameter count does not compensate for the lack of domain alignment: specialization yields greater efficiency, robustness, and transferability than sheer model size. Domain-specialized pretraining on homogeneous, high-resolution 2D mammography data, therefore, produces stronger alignment and superior generalization than heterogeneous, multi-modal training.

% These results demonstrate that domain-specialized pretraining on homogeneous, high-resolution 2D mammography data yields stronger alignment, greater robustness, and superior transfer than heterogeneous generalist pretraining.

Mammo-CLIP achieves superior performance through a set of key design principles. First, mammography is a dense, high-resolution modality where fine-grained texture and structural detail encode diagnostic signal. Generalist models, trained on low-resolution patches -- 896$\times$896 in MedGemma, 512$\times$512 in DINOv3 and 224$\times$224 in CXR-CLIP -- fail to capture the subtle morphological cues \eg, microcalcifications or architectural distortions. Mammo-CLIP processes mammograms at 1,520$\times$912 resolution, preserving diagnostic spatial detail essential for accurate interpretation. Second, pretraining across multiple institutions scales data diversity and substantially improves generalization. Third, Mammo-CLIP aligns real-world mammograms with their corresponding reports, producing cross-modal representations that transfer effectively across downstream tasks. This alignment drives strong zero-shot, linear probe, and fine-tuned performance on both in-distribution (EMBED) and out-of-distribution (VinDr) datasets. Despite training solely on screening exams without explicit cancer annotations, Mammo-CLIP generalizes to cancer classification on RSNA and EMBED, outperforming all generalist baselines. The model identifies visual patterns predictive of malignancy, enabling accurate cancer detection without retraining. These aligned visual representations also yield more accurate and interpretable prognosis than AsymMIRAI, which relies on a shallow ResNet-18 encoder. Even with the encoder frozen, Mammo-CLIP’s representations retain high semantic fidelity, demonstrating that strong visual priors directly translate to reliable risk prediction.

Leveraging these rich visual embeddings, Mammo-GRG, our report generation model, translates diagnostic understanding into structured clinical language and achieves superior performance over all generalist baselines through three key design choices. First, unlike generalist models that process individual images at low resolution, Mammo-GRG leverages the high-fidelity Mammo-CLIP vision encoder to handle large-scale mammograms to preserve subtle diagnostic features. Further, it encodes all four views with corresponding learnable positional embeddings and view-specific tokens (\texttt{\textless LCC\textgreater, \textless LMLO\textgreater, \textless RCC\textgreater, \textless RMLO\textgreater}) to maintain spatial relationships and laterality. Second, its language model, Llama 3.1-8B, is fine-tuned on question–answer pairs derived from real-world mammography reports, improving clinical specificity and contextual grounding. Third, a final grounding stage constrains generated text using Mammo-CLIP’s structured outputs, enforcing factual correctness, cross-view consistency, and diagnostic coherence. This integrated design produces reports with high lexical accuracy and clinical validity, reflecting expert radiologic reasoning, which the generalist models lack.

Despite these advances, our study has several limitations. First, the pretraining dataset, though multi-institutional, may inherit demographic or scanner biases that propagate through Mammo-CLIP and Mammo-GRG. Second, the risk predictor distills knowledge from MIRAI and may inherit latent biases from its teacher model. Third, zero-shot classification remains sensitive to prompt variation. Fourth, the performance of Mammo-GRG depends on the capabilities and alignment of its underlying large language model. Finally, our framework leverages only 2D mammograms; future work should extend this framework to 3D modalities such as digital breast tomosynthesis, CT, or MRI to capture volumetric context and temporal evolution of disease.

In summary, this work establishes that domain-specific foundation models achieve performance, interpretability, and clinical value beyond the reach of generalist models. Tailored image-text models like Mammo-CLIP and Mammo-GRG represent a clear path toward transparent, trustworthy, and scalable AI in medicine.

% points to be added:
% 1. hallucination - ref to prev report, stale nodule (limitation)
% 2. Trend on the baseline
% 3. Why UPMC reports have better performance than BU.
%  MIRAI w/ mammo-clip is better risk predictor because of transformer

==> sections/discussion_v3.tex <==
Mammo-CLIP (multi-institution) pretraining dataset leverages a large, multi-institutional corpus of 140,677 patients across UPMC, BU, Mayo Clinic, and EMBED -- four geographically and demographically diverse patient populations across the US. This diversity strengthens cross-domain generalization. To accommodate institutional privacy, the training protocol adopts a simple federated learning setup, alternating training epochs between a central server and the Mayo Clinic site. This protocol avoids the synchronization cost of more complex algorithms \eg FedAvg, which remain viable for future exploration. Our pretraining data consists of screening mammograms (BI-RADS 0, 1, and 2 only) and associated reports driving the model to learn the semantic precursors to malignancy -- \eg masses and calcifications -- directly from the text, learning a more nuanced diagnostic representation. Our Mammo-CLIP architecture addresses mammography’s unique visual and linguistic constraints. The EfficientNet-B5 backbone supports higher resolution $1520 \times 912$ mammograms, retaining the fine structural details essential for diagnosis \eg calcifications. The ModernBERT text encoder accommodates the long-form structure of radiology reports (mean 74 tokens, max 505) without truncation, preserving both local and contextual semantics. Also, we initialize the language encoder of Mammo-CLIP by finetuning on $\sim200k$ chest CT radiology reports, substantially enhancing multimodal alignment and downstream clinical performance.

% Data Efficiency and Generalizability:
Mammo-CLIP demonstrates strong generalization across both ID (EMBED) and OOD (RSNA and VinDr) datasets.
Mammo-CLIP multi-institutional variant consistently exceeds the UPMC-only version by 13–15\% AUROC on average, confirming that diversity and scale in pre-training data strengthens feature generalization. Among the baselines, MedSigLIP's broad medical pre-training proves more effective than DINOv3's natural image data, while CXR-CLIP's narrow domain specialization performs worst. Our evaluation focuses on mass, calcification, and architectural distortion, as other findings have insufficient prevalence (\textless1\% prevalence). Across individual findings, calcification classification achieves the highest AUROC ( \textless 0.95), as calcifications present with distinct high-contrast morphology, consistent terminology in reports, and limited inter-case variability -- factors that facilitate robust visual–textual alignment. Full fine-tuning (only for 5 epochs) consistently surpasses linear probing, since end-to-end optimization enables deeper adaptation of both image and text representations to task-specific distributions. In both linear probing and full fine-tuning, Mammo-CLIP (multi-institution) trained on just 25\% of the data outperforms MedSigLIP trained on 80\%, achieving on average a 10–15\% relative AUROC gain, consistently across ID and OOD benchmarks and for all evaluated findings. Note that Mammo-CLIP image encoder is 10 times smaller than MedSigLIP image encoder($\sim$30M \vs400M parameters). This efficiency emerges from two design choices. First, Mammo-CLIP is pre-trained on the largest real-world mammography-report corpus to date, in contrast to MedSigLIP’s general medical corpus, DINOv3’s natural image data, and CXR-CLIP’s single-modality chest X-ray data. Second, its image encoder processes full-resolution mammograms ($1,520 \times 912$), preserving fine-scale diagnostic patterns -- \eg microcalcifications -- that lower-resolution models (MedSigLIP: $448 \times 448$; DINOv3: $512 \times 512$; CXR-CLIP: $224 \times 224$) fail to capture. 

% prognosis
Mammo-CLIP image encoder serves as a foundation for explainable breast cancer prognosis by aligning image and text representations within a shared semantic space. The SOTA risk model MIRAI does not offer textual interpretability because its visual encoders lack language alignment. MIRAI w/ Mammo-CLIP and AsymMIRAI w/ Mammo-CLIP both achieve high-fidelity risk prediction while, for the first time, enabling text-based and image-based interpretability. For post hoc concept-level interpretation, we employ a Matryoshka Sparse Autoencoder (SAE) rather than a handcrafted asymmetry-based design. SAE retains the expressivity of the original predictor (Fig.~\ref{fig:prognosis}h) and exposes neuron-level semantics without constraining the model’s latent space. This framework, for the first time, grounds visual activations in corresponding radiology report sentences, enabled by Mammo-CLIP’s shared image–text embedding space. Our Mammo-CLIP-based risk predictors are trained using knowledge distillation from MIRAI, which is trained on large-scale cancer datasets and encodes robust malignancy patterns. In contrast, Mammo-CLIP is pretrained on screening mammograms without explicit cancer supervision. This distillation transfers MIRAI’s prognostic malignancy signal into Mammo-CLIP-based risk predictors while retaining the latter’s image-text alignment. Between the two variants, MIRAI w/ Mammo-CLIP surpasses AsymMIRAI w/ Mammo-CLIP due to its transformer-based aggregation of multi-view features and concurrent training across all risk horizons.


% report generation
Evaluating medical report generation remains a major challenge, as conventional linguistic metrics such as BLEU and ROUGE capture lexical overlap but ignore clinical accuracy. Therefore, for the first time, we adapt the GREEN framework, using an LLM judge (GPT-40-mini) to quantify mammography-specific clinical factuality and serve as a stronger benchmark for radiology report assessment. Mammo-GRG, the first multi-view report generator for mammography, outperforms all generalist baselines by achieving $\textgreater$55\%  higher GREEN scores than the fine-tuned generalist model MedGemma. Mammo-GRG on UPMC consistently performs better than on BU, due to richer linguistic structure and longer contextual descriptions in UPMC reports (mean sentences 47.5 in UPMC  \vs 32.1 in BU, refer to Fig.~\ref{fig:app_report_stats}). Such performance improvement is driven by explicit architectural and data-level design. First, Mammo-GRG is instruction-tuned on 359,746 QA pairs derived from real-world mammography reports across UPMC and BU, providing task-specific supervision that captures breast-imaging semantics instead of generic medical language. Second, unlike the baselines, our Mammo-CLIP vision encoder processes all four high-resolution ($1520 \times 912$) views simultaneously, using view-specific tokens and positional embeddings, mirroring the clinical reasoning process. Finally, Mammo-GRG integrates Mammo-CLIP’s high-fidelity vision–language representations for factual verification (refer to Fig.~\ref{fig:app_Mammo_GRG_grounding} for the effect of Mammo-CLIP's zero-shot grounding on Mammo-GRG), ensuring generated findings remain anatomically and clinically consistent. 


% limnitation:
Despite these advances, our study has several limitations. First, the pretraining dataset, though multi-institutional, may inherit demographic or scanner biases that propagate through Mammo-CLIP and Mammo-GRG. Second, the risk predictor distills knowledge from MIRAI and may inherit latent biases from its teacher model. Third, zero-shot classification remains sensitive to prompt variation. Fourth, the performance of Mammo-GRG depends on the capabilities and alignment of its underlying large language model (LLM). The LLM occasionally hallucinates findings or misinterprets stable lesions that depend on prior comparisons that are absent from the current input. Finally, our framework leverages only 2D mammograms; future work should extend this framework to 3D modalities such as digital breast tomosynthesis, CT, or MRI to capture volumetric context and temporal evolution of disease.

In summary, this work establishes that domain-specific foundation models achieve performance, interpretability, and clinical value beyond the reach of generalist models. Tailored image-text models like Mammo-CLIP and Mammo-GRG represent a clear path toward transparent, trustworthy, and scalable AI in medicine.

 % points to be added:
% 1. hallucination - ref to prev report, stale nodule (limitation)


==> sections/introduction_v1.tex <==

% Breast cancer is most important form - its deadly. \cite{bray2024global} % Mention the death of cancer and mention the age. (\cite{giaquinto2024breast})
% Diagnosis: Why {including high false-positive rates and lower sensitivity for women with dense breast tissue} rate of mis diagnosis (\cite{khan2025advances, nelson2016factors, lehman2017national})
% overdiagnosis - This can lead to unnecessary treatments, including surgery, radiation, and hormonal therapies, which carry their own risks and side effects {\cite{ryser2022estimation}}
% Misdiagnosis can also occur at the pathology level.

% Prognosis: If is doagnosed earlier , this much life will be saved (\cite{nicholson2024screening, trentham2024collaborative, duffy2010absolute, duffy2020effect})
% women aobve age are asked to come to scanner , and this create this much of risk
% Motivate: Woman above X come to screening. They possess having more risk. Mammo screening/per yr (woman after X goes to screening.)
% In the US, after 40-50 these people need to do screening. \cite{nicholson2024screening}
%  this increases the load to radiologist (cite) - chances for misdiagnosis due to this load. \cite{alshabibi2020impact, stec2018systematic, kwee2021workload, dodelzon2024factors}
% We need to do a prognosis well. So, we need to priorotize. 
% If diagnosis earlier, lots of lives can be saved  
% In AI, MIRAI (\cite{yala2022multi}) does prognosis but MIRAI is not interpretable. why interpretability matters in AI (\cite{rezazade2023impact, singh2020explainable, salahuddin2022transparency})
% Also radiologist spend a lot of time in taking notes. This creates burden (\cite{glover2017quantifying, dhanoa2013evolving} ), so we need a FM for mammo which will do prognosis and report gen to mitigate the gap.


%  put numbers - very general and needs direct
% Breast cancer remains a leading cause of cancer-related mortality among women globally\cite{bray2024global}, with risk and incidence increasing significantly with age \cite{giaquinto2024breast}. Detecting cancer at an early stage substantially improves patient outcomes and saves lives \cite{nicholson2024screening, trentham2024collaborative, duffy2010absolute, duffy2020effect}. However, screening mammography presents significant diagnostic challenges. First, it is limited by high false-positive rates and reduced sensitivity in women with dense breast tissue \cite{khan2025advances, nelson2016factors, lehman2017national}. Second, it carries a substantial risk of overdiagnosis, a practice that exposes patients to avoidable surgery, radiation, and endocrine therapy \cite{ryser2022estimation}. In the United States, guidelines now recommend routine screening for women beginning at age 40, greatly expanding the asymptomatic population undergoing imaging \cite{nicholson2024screening}. This surge in volume increases radiologist workload and decision fatigue, which correlates with variable performance and missed cancers \cite{alshabibi2020impact, stec2018systematic, kwee2021workload, dodelzon2024factors}. Risk-stratified prognosis is therefore needed to prioritize reading queues and personalize patient follow-up. Recent AI systems such as MIRAI provide multi-year risk prediction but offer limited interpretability for clinical auditing \cite{yala2022multi}. Concurrently, radiologists spend considerable time authoring structured reports, a task which compounds existing throughput pressures \cite{glover2017quantifying, dhanoa2013evolving}. We therefore motivate a foundation model for mammography that unifies prognostic inference with report generation. Our goal is to deliver calibrated, interpretable risk estimates that reduce documentation burden, enhance clinical triage, and support scalable, equitable screening.

% *  Different ways of training FM -- however multimodal (specifially contrastive Vision text) are successfull b/c text provided inexpesive and scalable supervision to learn impotant visual feature.
% * Motivation for FM for breast: - 1. Motivation for text, 2. Motivation of zeroshot and training with limited data and 3. Robustness 4. Interpretability.
% * Motivation for text: Importance of text from radiology report provide extra signal or supervision. This is inexpensive and scalable
% * For ex, density or calcification - which is important to diagnose cancer (\cite{boyd2007mammographic, kim2022microcalcifications, azam2021mammographic}) -  in breast mammo often show up in the radiology report - those can bootstrap AI mnodel for diagnosis and prognosis
% * Motivation of zeroshot and training with limited data: Since collecting large scale dataset with annotaiton in healthcare domain are cost prohibitive, FM have the advantage by providing data efficiency (they showcase great Zero shot performance) b/c a model can be fine tuneed for a new purpuse or for new site with limmited data.
% * Robustness: Next issue is out of distribution robustness, for example a model that is trained for one health system can be transferred with no or limmited fine tuning to dataset from other hospital. Previous studies have shown that the most important predictor of the robustness of the AI model is the same size. Creating large-scale sample size for different tasks (ie prognosis , diagnosis and report genration) is even more cost prohibitive. This is another motivation for FM, namely if we can create one robust model that can be trained on large scale dataset and excell on multiple tasks then we acheive robustness. Such model can also be used as effective retrival model (zero shot) which can also be helpful for retriveling similar patients (ie helping clinical for differential diagnosis).
% * building a model on the top of a model where image and text are aligned can provide exlaibability for free 
%  Text can be used for interpretability: \cite{varma2023villa, zhong2022regionclip}, localize a disease


% Use first, second, third a nice coherence.
% Multimodal foundation models achieve remarkable success by using vision-language pretraining~\cite{radford2021learning, zhang2020contrastive, huang2021gloria, wu2023medklip, wang2022medclip}, where text provides an inexpensive and scalable supervisory signal for learning semantically rich visual representations. This paradigm is especially well-suited for mammography. Radiology reports routinely document key prognostic indicators, such as mammographic density, microcalcifications \etc, which are established as independent risk factors for breast cancer \cite{boyd2007mammographic, kim2022microcalcifications, azam2021mammographic}. These clinical texts can bootstrap a model's reasoning of both diagnostic and prognostic features. Foundation models also address the challenge of data scarcity in medicine, where creating large-scale annotated datasets is cost-prohibitive. Their data efficiency manifests as strong zero-shot and few-shot performance, enabling adaptation to new tasks or clinical sites with limited labeled data. Furthermore, a unified foundation model offers a step toward out-of-distribution robustness. A single model trained on a massive, diverse dataset exhibits a degree of generalization across multiple downstream tasks and healthcare systems that is difficult to achieve with smaller, task-specific models. Such a model can also function as a zero-shot retrieval engine to find clinically similar precedent cases. Finally, pretraining on paired image regions and text provides a direct path to interpretability. This alignment allows the model to localize and ground its textual descriptions in the image, a critical feature for clinical auditing and trust \cite{varma2023villa, zhong2022regionclip}.


In 2022, breast cancer accounted for 2.3 million new cases and 666,000 deaths globally, making it the most diagnosed cancer worldwide \cite{bray2024global}. Detecting the disease at an early stage is critical; screening women from age 40 has been shown to reduce breast cancer mortality by 25\% over 10 years \cite{duffy2020effect, trentham2024collaborative}. However, screening mammography presents significant diagnostic challenges. First, screening mammography exhibits two critical limitations: high recall rates (averaging 11.5\% nationally in the U.S.) and substantially reduced sensitivity in women with dense breast tissue \cite{lehman2017national, nelson2016factors}. Second, overdiagnosis poses a substantial risk, estimated at 15\% of screen-detected cancers. This risk directly exposes patients to avoidable surgery, radiation, and endocrine therapy \cite{ryser2022estimation}. 
Third, the expanding screening guidelines in the United States now include routine imaging for women beginning at age 40, dramatically increasing the asymptomatic population undergoing mammography \cite{nicholson2024screening}.
This surge in volume intensifies workload pressures on radiologists, whose clinical time remains finite. Up to 44\% of their workday involves non-interpretive tasks such as documentation and communication, compounding cognitive fatigue and driving diagnostic errors \cite{glover2017quantifying, stec2018systematic, kwee2021workload}. 
These limitations underscore the need for AI-driven solutions that integrate diagnosis, prognosis, and automated report generation. Foundation models offer a natural framework for this goal. Through large-scale pretraining, they learn robust, generalizable mammographic representations that capture both anatomical and pathological variation. Such transferable representations can support diverse downstream tasks: high-specificity diagnosis, multi-year risk prediction, and automated report generation. Building on this principle, this paper introduces a domain-specific foundation model for mammography that delivers calibrated, interpretable risk estimates to triage reading queues, provides robust diagnostic support, and automates structured report generation. This unified approach reduces documentation burden, enhances clinical triage, and provides the necessary infrastructure for scalable, equitable screening.

% Risk-stratified prognosis is therefore needed to prioritize reading queues and personalize patient follow-up. While recent AI systems such as MIRAI~\cite{yala2022multi} can predict multi-year risk with an AUC of 0.75, they offer limited interpretability for clinical auditing \cite{rezazade2023impact, salahuddin2022transparency}. This paper aims to address the gap by developing a foundation model for mammography that unifies prognostic inference with report generation. Our goal is to deliver calibrated, interpretable risk estimates that reduce documentation burden, enhance clinical triage, and support scalable, equitable screening.

% In the United States, guidelines now recommend routine screening for women beginning at age 40, greatly expanding the asymptomatic population undergoing imaging \cite{nicholson2024screening}. This surge in volume places an immense burden on radiologists, whose time is already constrained. Radiologists spend a considerable portion of their day on non-interpretive tasks, with clinical documentation and communication comprising up to 44\% of their daily workload, which compounds decision fatigue and correlates with diagnostic errors \cite{glover2017quantifying, stec2018systematic, kwee2021workload}. 




Multimodal foundation models achieve remarkable success in computer vision by using vision-language pretraining~\cite{radford2021learning, zhang2020contrastive, huang2021gloria, wu2023medklip, wang2022medclip}, where text provides an inexpensive and scalable supervisory signal for learning semantically rich visual representations. This paradigm is uniquely suited to address the challenges in mammography for four key reasons. First, radiology reports routinely document key prognostic indicators, such as breast density, microcalcifications \etc, as independent risk factors for breast cancer \cite{boyd2007mammographic, kim2022microcalcifications, azam2021mammographic}. These clinical texts can bootstrap a model's reasoning of both diagnostic and prognostic features. Second, foundation models also address the challenge of data scarcity in medicine, where creating large-scale annotated datasets is cost-prohibitive. Leveraging pretraining scale, they achieve strong zero-shot and linear probe performance, enabling adaptation to new clinical tasks and sites with minimal labeled data. Third, a unified foundation model offers a step toward out-of-distribution robustness. A single foundation model trained on large, heterogeneous data achieves broad generalization across tasks and healthcare systems, surpassing the robustness of smaller task-specific models. Finally, pretraining on paired image regions and text provides a direct path to interpretability. This alignment allows the model to localize and ground its textual descriptions in the image, a critical feature for clinical auditing and trust \cite{varma2023villa, zhong2022regionclip}.


% Such a model can also function as a zero-shot retrieval engine to find clinically similar precedent cases. 

One potential strategy is to construct robust vision–language models for mammography using generalist models, \eg MedGemma~\cite{sellergren2025medgemma} and its vision encoder MedSigLIP, or from models pre-trained on large datasets from other imaging modalities, \eg chest X-rays~\cite{huang2021gloria, wu2023medklip, wang2022medclip}. However, these methods have fundamental limitations. First, generalist models often operate on downsampled images or low-resolution patches (MedSigLip uses $448\times448$ image resolution), a strategy that fails to capture subtle, diagnostically critical features unique to mammography \eg microcalcifications and architectural distortions. Second, these models exhibit poor data efficiency and zero-shot performance when transferred to the high-resolution and fine-grained mammography domain. These limitations motivate a domain-specific approach guided by four core desiderata. First, the model must operate on high-resolution images to preserve the fine-grained pathological details. Second, it must handle the inherent heterogeneity of real-world clinical data, including datasets with missing reports, partial annotations, or incomplete imaging views from multiple institutions. Third, its effectiveness must be evaluated across a comprehensive suite of clinical applications, including diagnosis, prognosis, report generation, and pathology localization. Finally, the model must demonstrate robustness against the dataset shifts -- generalizing reliably to unseen institutions, imaging devices, and patient demographics -- commonly encountered when deploying in new clinical environments.


% Overview of the method [similar to Sun-In Lee [paper]
% This needs a rewrite

\begin{figure}[p]
    \centering
    % \includegraphics[height=0.8\textheight]{figures/main.pdf}
    \includegraphics[width=0.92\textwidth]{figures/main.pdf}
    \vspace{-0.8em}
    \caption{\textbf{Overview of the Mammo-CLIP foundation model and downstream applications.} \textbf{a.} Schematic of the Mammo-CLIP framework. High-resolution mammographic views (CC, MLO) and paired radiology reports are jointly used for multi-view contrastive pretraining, aligning image and text representations within a shared embedding space (see Methods). \textbf{b.} Composition of multi-institutional pretraining datasets from the Mayo Clinic, BU, UPMC, and EMBED cohorts. \textbf{c.} Composition of evaluation datasets used to benchmark diagnostic and prognostic generalization across in-distribution (ID; EMBED) and out-of-distribution (OOD; RSNA, VinDr) settings. \textbf{d.} Pathology localization by integrating the Mammo-CLIP vision encoder into a RetinaNet detector. \textbf{e.} Zero-shot classification with Mammo-CLIP. Image and text encoders map mammograms and prompts into a shared space. Similarity between embeddings enables classification without fine-tuning. \textbf{f.} Findings classification under either linear-probe or full fine-tuning settings where a linear classifier is attached to Mammo-CLIP image encoder, quantifying the quality of the learned visual representations. \textbf{g.} Interpretable risk prediction built on the AsymMIRAI framework using frozen Mammo-CLIP encoders to compute bilateral asymmetry across CC and MLO views for 1–5 year risk estimation. \textbf{h.} Automated report generation (Mammo-GRG) combining Mammo-CLIP with a Llama-3.1-8B language model to produce clinically grounded radiology reports.}  
    \label{fig:schematic}
\end{figure}


\begin{table*}[t]
\centering
\footnotesize
\begin{threeparttable}
\caption{Summary characteristics of the EMBED, UPMC, and Mayo Clinic datasets used to pre-train Mammo-CLIP. Note that the Mammo-GRG pretraining also leverages the same UPMC dataset. }
\label{tab:main_dataset_char}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{5pt}

\begin{tabularx}{\textwidth}{l l Y Y Y}
\rowcolor{nmHeader}
\textbf{\color{nmHeadTxt} Characteristic} &
\textbf{\color{nmHeadTxt} Category} &
\textbf{\color{nmHeadTxt} EMBED (N=20,381)} &
\textbf{\color{nmHeadTxt} UPMC (N=13{,}829)} &
\textbf{\color{nmHeadTxt} Mayo Clinic (N=96{,}567)} \\

\midrule

\multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{BI-RADS}} &
0 & 5{,}476 (15.4\%) & 2{,}125 (15.4\%) & \NA \\
& 1 & 10{,}822 (31.7\%) & 4{,}376 (31.7\%) & \NA \\
& 2 & 4{,}083 (52.9\%) & 7{,}328 (52.9\%) & \NA \\
\addlinespace[3pt]\midrule

\multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Age Group}} &
$<$ 50 years & 956 (9.6\%) & 1{,}326 (9.6\%) & 2{,}476 (2.4\%) \\
& 50–60 years & 11{,}163 (44.6\%) & 6{,}163 (44.6\%) & 45{,}513 (47.3\%) \\
& $>$ 60 years & 8{,}262 (45.8\%) & 6{,}340 (45.8\%) & 48{,}578 (50.4\%) \\
\addlinespace[3pt]\midrule

\multirowcell{4}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Breast Density}} &
Almost entirely fatty (A) & 3{,}113 (22.5\%) & 6{,}159 (22.5\%) & 9{,}712 (10.0\%) \\
& Scattered fibroglandular (B) & 5{,}712 (41.3\%) & 5{,}233 (41.3\%) & 47{,}370 (49.0\%) \\
& Heterogeneously dense (C) & 3{,}801 (27.5\%) & 6{,}765 (27.5\%) & 34{,}861 (36.1\%) \\
& Extremely dense (D) & 1{,}203 (8.7\%) & 2{,}224 (8.7\%) & 4{,}624 (4.9\%) \\
\addlinespace[3pt]\midrule

\multirowcell{4}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Race}} &
Black & 8{,}580 (42.1\%) & \NA & 893 (0.9\%) \\
& White & 8{,}193 (40.2\%) & \NA & 92{,}287 (95.3\%) \\
& Asian & 1{,}305 (6.4\%) & \NA & 1{,}713 (1.7\%) \\
& Other & 2{,}303 (11.3\%) & \NA & 1{,}674 (1.7\%) \\
\addlinespace[3pt]\midrule

\multirowcell{5}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Manufacturer}} &
HOLOGIC, Inc. & \NA & 13{,}443 (96.7\%) & 90{,}351 (93.5\%) \\
& LORAD & \NA & 287 (2.1\%) & 1{,}359 (1.5\%) \\
& SIEMENS & \NA & 99 (0.7\%) & 5 ($<$0.1\%) \\
& Visage & \NA & \NA & 20 ($<$0.1\%) \\
& Unknown & \NA & \NA & 4{,}832 (5.0\%) \\

\bottomrule
\end{tabularx}

\begin{tablenotes}[flushleft]\footnotesize
\item \textbf{Note:} Missing entries are indicated by \NA. BI-RADS categories follow standard clinical grading; percentages are computed relative to total patient count.
\end{tablenotes}
\end{threeparttable}
\end{table*}


% \begin{table*}[t]
% \centering
% \footnotesize
% \begin{threeparttable}
% \caption{Summary characteristics of the EMBED dataset, used to pre-train Mammo-CLIP and Mammo-GRG.}
% \label{tab:bu_dataset_characteristics}
% \renewcommand{\arraystretch}{1.15}
% \setlength{\tabcolsep}{5pt}

% \begin{tabularx}{\textwidth}{l l Y}
% \rowcolor{nmHeader}
% \textbf{\color{nmHeadTxt} Characteristic} &
% \textbf{\color{nmHeadTxt} Category} &
% \textbf{\color{nmHeadTxt} Count (\%)} \\

% \midrule

% \multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{BI-RADS}} &
% 0 & 5{,}476 (15.4\%) \\
% & 1 & 10{,}822 (31.7\%) \\
% & 2 & 4{,}083 (52.9\%) \\
% \addlinespace[3pt]\midrule

% \multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Age Group}} &
% $<$ 50 years & 956 (9.6\%) \\
% & 50–60 years & 11{,}163 (44.6\%) \\
% & $>$ 60 years & 8{,}262 (45.8\%) \\
% \addlinespace[3pt]\midrule

% \multirowcell{4}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Breast Density}} &
% Almost entirely fatty (A) & 3{,}113 (22.5\%) \\
% & Scattered fibroglandular (B) & 5{,}712 (41.3\%) \\
% & Heterogeneously dense (C) & 3{,}801 (27.5\%) \\
% & Extremely dense (D) & 1{,}203 (8.7\%) \\
% \addlinespace[3pt]\midrule

% \multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Race}} &
% Black & 8{,}580 (42.1\%) \\
% & White & 8{,}193 (40.2\%) \\
% & Asian & 1{,}305 (6.4\%) \\
% & Other & 2{,}303 (11.3\%) \\

% \bottomrule
% \end{tabularx}

% \begin{tablenotes}[flushleft]\footnotesize
% \item \textbf{Note:} BI-RADS categories follow standard clinical grading; percentages are computed relative to total patient count.
% \end{tablenotes}
% \end{threeparttable}
% \end{table*}


% \begin{table*}[h]
% \centering
% \footnotesize
% \begin{threeparttable}
% \caption{Summary characteristics of the UPMC dataset. It is one of the pretraining datasets used to pre-train Mammo-CLIP and Mammo-GRG.}
% \label{tab:bu_dataset_characteristics}
% \renewcommand{\arraystretch}{1.15}
% \setlength{\tabcolsep}{5pt}

% \begin{tabularx}{\textwidth}{l l Y}
% \rowcolor{nmHeader}
% \textbf{\color{nmHeadTxt} Characteristic} &
% \textbf{\color{nmHeadTxt} Category} &
% \textbf{\color{nmHeadTxt} Count (\%)} \\

% \midrule

% \multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{BI-RADS}} &
% 0 & 2{,}125 (15.4\%) \\
% & 1 & 4{,}376 (31.7\%) \\
% & 2 & 7{,}328 (52.9\%) \\
% \addlinespace[3pt]\midrule

% \multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Age Group}} &
% $<$ 50 years & 1{,}326 (9.6\%) \\
% & 50–60 years & 6{,}163 (44.6\%) \\
% & $>$ 60 years & 6{,}340 (45.8\%) \\
% \addlinespace[3pt]\midrule

% \multirowcell{4}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Breast Density}} &
% Almost entirely fatty (A) & 6{,}159 (22.5\%) \\
% & Scattered fibroglandular (B) & 5{,}233 (41.3\%) \\
% & Heterogeneously dense (C) & 6{,}765 (27.5\%) \\
% & Extremely dense (D) & 2{,}224 (8.7\%) \\
% \addlinespace[3pt]\midrule

% \multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Manufacturer}} &
% HOLOGIC, Inc. & 13{,}443 (96.7\%) \\
% & LORAD & 287 (2.1\%) \\
% & SIEMENS & 99 (0.7\%) \\

% \bottomrule
% \end{tabularx}

% \begin{tablenotes}[flushleft]\footnotesize
% \item \textbf{Note:} BI-RADS categories follow standard clinical grading; percentages are computed relative to total patient count.
% \end{tablenotes}
% \end{threeparttable}
% \end{table*}


% \begin{table*}[h]
% \centering
% \footnotesize
% \begin{threeparttable}
% \caption{Summary characteristics of the Mayo Clinic dataset used to pretrain Mammo-CLIP. Values represent patient-level counts with percentages shown in parentheses.}
% \label{tab:mammo_clip_pretrain_characteristics}
% \renewcommand{\arraystretch}{1.15}
% \setlength{\tabcolsep}{5pt}

% \begin{tabularx}{\textwidth}{l l Y}
% \rowcolor{nmHeader}
% \textbf{\color{nmHeadTxt} Characteristic} &
% \textbf{\color{nmHeadTxt} Category} &
% \textbf{\color{nmHeadTxt} Count (\%)} \\

% \midrule
% % \multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Age at screening}} &
% % Median (y) & 56 & 62 \\
% % & Range (y) & 24--87 & 34--87 \\
% % \addlinespace[3pt]\midrule

% \multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Age Groups}} &
% $<$ 40 y & 2{,}476 (2.4\%) \\
% & 40–60 y & 45{,}513 (47.3\%) \\
% & 60–89 y & 48{,}578 (50.4\%) \\
% \addlinespace[3pt]\midrule

% \multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Race}} &
%  White & 92{,}287 (95.3\%) \\
% & Asian & 1{,}713 (1.7\%) \\
% & Black & 893 (0.9\%) \\
% & Other & 1{,}674 (1.7\%) \\
% \addlinespace[3pt]\midrule

% \multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Density}} &
%  A & 9{,}712 (10.0\%) \\
% & B & 47{,}370 (49.0\%) \\
% & C & 34{,}861 (36.1\%) \\
% & D & 4{,}624 (4.9\%) \\
% \addlinespace[3pt]\midrule

% \multirowcell{4}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Manufacturer}} &
% HOLOGIC, Inc. & 90{,}351 (93.5\%) \\
% & LORAD & 1{,}359 (1.5\%) \\
% & Visage & 20 ($<$0.1\%) \\
% & SIEMENS & 5 ($<$0.1\%) \\
% & Unknown & 4{,}832 ($5.0\%$) \\
% \addlinespace[3pt]\midrule

% % \multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{1-year Cancer}} &
% % Negative (0) & 94{,}896 (98.3\%) \\
% % & Positive (1) & 1{,}671 (1.7\%) \\
% % \addlinespace[3pt]\midrule

% % \multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{2-year Cancer}} &
% % Negative (0) & 94{,}601 (99.7\%) \\
% % & Positive (1) & 295 (0.3\%) \\
% % \addlinespace[3pt]\midrule

% % \multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{3-year Cancer}} &
% % Negative (0) & 94{,}371 (99.8\%) \\
% % & Positive (1) & 230 (0.2\%) \\
% % \addlinespace[3pt]\midrule

% % \multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{4-year Cancer}} &
% % Negative (0) & 94{,}149 (99.8\%) \\
% % & Positive (1) & 222 (0.2\%) \\
% % \addlinespace[3pt]\midrule

% % \multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{5-year Cancer}} &
% % Negative (0) & 93{,}905 (99.7\%) \\
% % & Positive (1) & 244 (0.3\%) \\

% % \bottomrule
% \end{tabularx}

% \begin{tablenotes}[flushleft]\footnotesize
% \item \textbf{Note:} Cancer cases indicate exams followed by a confirmed diagnosis within the specified follow-up period.
% \end{tablenotes}
% \end{threeparttable}
% \end{table*}



\begin{table*}[t]
\centering
\footnotesize
\begin{threeparttable}
\caption{Characteristics of BU datasets. It consists of 54,776 screening images from 9,900 patients and 13,480 exams with complete data, that includes an associated radiology report and followup data on clinical outcomes. It is one of the pretraining datasets used to pre-train Mammo-CLIP and Mammo-GRG. Among the 1,041 total cancer cases, the number of cases occurring within years 1–5 are 283, 212, 205, 188, and 153, respectively.}
\label{tab:bu_dataset_characteristics}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{5pt}

\begin{tabularx}{\textwidth}{l l Y Y}
\rowcolor{nmHeader}
\textbf{\color{nmHeadTxt} Characteristic} &
\textbf{\color{nmHeadTxt} Category} &
\textbf{\color{nmHeadTxt} All} &
\textbf{\color{nmHeadTxt} Cases} \\
\midrule

\rowcolor{nmSubhdr}\textbf{Exams} &  & 13{,}480 & 1{,}041 \\
\addlinespace[3pt]\midrule

\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Age at screening}} &
Median (y) & 56 & 62 \\
& Range (y) & 24--87 & 34--87 \\
\addlinespace[3pt]\midrule

\multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Age groups}} &
$<$ 50 y & 3{,}878 (28.7\%) & 114 (10.9\%) \\
& 50--70 y & 7{,}990 (59.3\%) & 747 (71.8\%) \\
& $>$ 70 y & 1{,}617 (12.0\%) & 180 (17.3\%) \\
\addlinespace[3pt]\midrule

\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Family history of breast cancer.}} &
 No & 12{,}950 (96.1\%) & 930 (89.3\%) \\
& Yes & 530 (3.9\%) & 111 (10.7\%) \\
\addlinespace[3pt]\midrule

\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{History of breast biopsy}} &
 No prior biopsy & 12{,}901 (95.7\%) & 922 (88.6\%) \\
& Prior biopsy, benign dx unknown & 579 (4.3\%) & 119 (11.4\%) \\
\addlinespace[3pt]\midrule

\multirowcell{5}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Mammographic density}} &
 Almost entirely fatty (A) & 3{,}428 (25.4\%) & 190 (18.3\%) \\
& Scattered fibroglandular (B) & 4{,}792 (35.6\%) & 524 (50.3\%) \\
& Heterogeneously dense (C) & 3{,}824 (28.3\%) & 268 (25.7\%) \\
& Extremely dense (D) & 1{,}323 (9.8\%) & 50 (4.8\%) \\
& Unknown & 113 (0.8\%) & 9 (0.9\%) \\
\addlinespace[3pt]\midrule

\multirowcell{4}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{BI-RADS}} &
 0 & 1{,}333 (9.9\%) & 319 (30.6\%) \\
& 1 & 11{,}062 (82.1\%) & 620 (59.6\%) \\
& 2 & 1{,}053 (7.8\%) & 81 (7.8\%) \\
& Other & 32 (0.2\%) & 21 (2.0\%) \\
\addlinespace[3pt]\midrule

% \multirowcell{5}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Final BI-RADS}} &
%  1 & 11{,}479 (85.1\%) & 637 (61.2\%) \\
% & 2 & 1{,}308 (9.7\%) & 112 (10.8\%) \\
% & 3 & 341 (2.6\%) & 26 (2.5\%) \\
% & 4--5 & 294 (2.2\%) & 189 (18.1\%) \\
% & Other & 58 (0.4\%) & 53 (5.1\%) \\
% \addlinespace[3pt]\midrule

\multirowcell{6}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Race and ethnicity}} &
 Black & 7{,}224 (53.6\%) & 557 (53.5\%) \\
& White & 2{,}573 (19.1\%) & 185 (17.8\%) \\
& Hispanic & 3{,}219 (23.9\%) & 251 (24.1\%) \\
& Asian & 327 (2.4\%) & 31 (3.0\%) \\
& Native American & 31 (0.2\%) & 3 (0.3\%) \\
& Unknown & 106 (0.8\%) & 14 (1.3\%) \\

\bottomrule
\end{tabularx}

\begin{tablenotes}[flushleft]\footnotesize
\item \textbf{Note:} Percentages are relative to the row’s population (\textbf{All} or \textbf{Cases}). Cases denotes \textbf{cancer cases}. Abbreviations: dx, diagnosis. Family history of breast cancer denotes cancer in first-degree relative(s).
\end{tablenotes}
\end{threeparttable}
\end{table*}


\begin{table*}[p]
\centering
\footnotesize
\begin{threeparttable}
\caption{Characteristics of evaluation datasets used to assess Mammo-CLIP’s image representations. Each dataset is \textbf{publicly} available. Each dataset corresponds to a distinct patient cohort: EMBED (N = 8,481), VinDr (N = 5,000), and RSNA (N = 11,913). Values are reported as patient counts (N) and percentages (\%). These datasets serve as diverse evaluation benchmarks for testing the generalizability and robustness of Mammo-CLIP’s image–text representations.}
\label{tab:dataset_eval_characteristics}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{5pt}

\begin{tabularx}{\textwidth}{l l Y Y Y}
% ====== Header (two rows: dataset names + locations) ======
\rowcolor{nmHeader}
\textbf{\color{nmHeadTxt} Characteristic} &
\textbf{\color{nmHeadTxt} Category} &
\textbf{\color{nmHeadTxt} EMBED (N=8,481)} &
\textbf{\color{nmHeadTxt} VinDr (N=5,000)} &
\textbf{\color{nmHeadTxt} RSNA (N=11,913)} \\
\rowcolor{nmHeader}
\textbf{\color{nmHeadTxt}} & \textbf{\color{nmHeadTxt}Location} &
\textcolor{nmHeadTxt}{Emory, GA, USA} &
\textcolor{nmHeadTxt}{Vietnam} &
\textcolor{nmHeadTxt}{USA} \\
\rowcolor{nmHeader}
\textbf{\color{nmHeadTxt}} & \textbf{\color{nmHeadTxt}\#Images} &
\textcolor{nmHeadTxt}{45{,}736} &
\textcolor{nmHeadTxt}{20{,}486} &
\textcolor{nmHeadTxt}{54{,}706} \\

\midrule

% --- Cancer ---
\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Cancer}} &
\textbf{Present} & \textbf{333 (3.9\%)} & \textbf{481 (9.6\%)} & \textbf{486 (4.1\%)} \\
& Absent & 8{,}148 (96.1\%) & 4{,}519 (90.4\%) & 11{,}427 (95.9\%) \\
\addlinespace[3pt]\midrule

% --- Mass ---
\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Mass}} &
\textbf{Present} & \textbf{1{,}588 (18.7\%)} & \textbf{584 (11.7\%)} & \NA \\
& Absent & 6{,}893 (81.3\%) & 4{,}416 (88.3\%) & \NA \\
\addlinespace[3pt]\midrule

% --- Calcification ---
\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Calcification}} &
\textbf{Present} & \textbf{1{,}435 (16.9\%)} & \textbf{220 (4.4\%)} & \NA \\
& Absent & 7{,}046 (83.1\%) & 4{,}780 (95.6\%) & \NA \\
\addlinespace[3pt]\midrule

% --- Architectural Distortion ---
\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Architectural Distortion}} &
\textbf{Present} & \textbf{183 (2.2\%)} & 65 (1.3\%) & \NA \\
& Absent & 8{,}298 (97.8\%) & 4{,}935 (98.7\%) & \NA \\
\addlinespace[3pt]\midrule

% --- Asymmetry ---
\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Asymmetry}} &
\textbf{Present} & \textbf{1{,}841 (21.7\%)} & 96 (2\%) & \NA \\
& Absent & 6{,}640 (78.3\%) & 4{,}904 (98.0\%) & \NA \\
\addlinespace[3pt]\midrule

% --- Nipple_Retraction ---
\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Nipple Retraction}} &
\textbf{Present} & \NA & 22 (0.5\%) & \NA \\
& Absent & \NA & 4{,}978 (99.5\%) & \NA \\
\addlinespace[3pt]\midrule

% --- Skin_Retraction  ---
\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Skin Retraction }} &
\textbf{Present} & \NA & 13 (0.2\%) & \NA \\
& Absent & \NA & 4{,}987 (99.8\%) & \NA \\
\addlinespace[3pt]\midrule

% --- Skin Thickening   ---
\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Skin Thickening  }} &
\textbf{Present} & \NA & 34 (0.7\%) & \NA \\
& Absent & \NA & 4{,}966 (99.3\%) & \NA \\
\addlinespace[3pt]\midrule

% --- Suspicious Lymph Node ---
\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Suspicious Lymph Node }} &
\textbf{Present} & \NA & 53 (1\%) & \NA \\
& Absent & \NA & 4{,}947 (99.0\%) & \NA \\
\addlinespace[3pt]\midrule

% --- BI-RADS ---
\multirowcell{6}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{BI\mbox{-}RADS}} 
& 0 & 133 (1.6\%) & \NA & 3{,}287 (27.5\%) \\
& 1 & 2{,}117 (25.0\%) & 2{,}515 (50.3\%) & 3{,}151 (26.4\%) \\
& 2 & 3{,}057 (36.0\%) & 1{,}568 (31.4\%) & 604 (5.07\%) \\
& 3 & 1{,}719 (20.3\%) & 436 (8.7\%) & \NA \\
& 4 & 1{,}262 (14.9\%) & 368 (7.4\%) & \NA \\
& 5 & 193 (2.27\%) & 113 (2.3\%) & \NA \\
\addlinespace[3pt]\midrule

% --- Race ---
\multirowcell{6}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Race}} 
& African American & 3{,}823 (45.2\%) & \NA & \NA \\
& Alaskan Native & 25 (0.3\%) &\NA& \NA \\
& Asian & 415 (4.9\%) & \NA & \NA \\
& Caucasian or White & 3{,}363 (39.8\%) & \NA & \NA \\
& Multiple & 39 (0.5\%) & \NA & \NA \\
& Native Hawaiian & 108 (1.3\%) &\NA & \NA \\
& Unreported & 680 (8.0\%) & \NA & \NA \\
\addlinespace[3pt]\midrule

% --- Density ---
\multirowcell{4}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Density}} &
Almost entirely fatty (A) & 133 (1.6\%) & 24 (0.48\%) & 553 (4.64\%) \\
& Scattered fibroglandular (B) & 2{,}117 (25.0\%) & 469 (9.37\%) & 2{,}511 (21.1\%) \\
& Heterogenously Dense (C) & 3{,}057 (36.0\%) & 3{,}826 (76.2\%) & 2{,}436 (20.4\%) \\
& Extremely Dense (D) & 1{,}719 (20.3\%) & 681 (13.6\%) & 309 (2.59\%) \\

\bottomrule
\end{tabularx}

\begin{tablenotes}[flushleft]\footnotesize
\item \textbf{Note:} \NA{} indicates data not available for that dataset. Bold values denote positive findings.
\end{tablenotes}
\end{threeparttable}
\end{table*}









% To address these challenges, this paper proposes Mammo-CLIP, a vision-language model specifically designed for mammography. Unlike existing approaches, Mammo-CLIP processes high-resolution 2D screening mammograms from real-world clinical cases, preserving fine diagnostic details essential for accurate interpretation. To improve generalization, Mammo-CLIP is pre-trained on 2D screening mammograms, learning transferable, fine-grained representations. Trained on a large, multi-centre dataset (N=195,976 studies) from the University of Pittsburgh Medical Center, Boston University, EMBED, and the Mayo Clinic, it achieves superior performance in both zero-shot and data-efficient settings.
% We pre-train Mammo-CLIP on a large corpus of 2D screening mammogram-report pairs and employ a dual strategy to learn robust representations. First, we augment the training data by synthesizing reports for mammograms that contain only mammographic attributes (\eg mass, calcification). Second, we utilize multi-view supervision (MVS) to learn generalizable features. On both in-distribution and out-of-distribution settings, we systematically evaluate the vision encoder's ability to identify critical mammographic findings -- including masses, calcifications, architectural distortion, and malignancy under zero-shot and data-efficiency settings using linear probes and full fine-tuning. We demonstrate the effectiveness of the Mammo-CLIP vision encoder on two challenging clinical applications. First, we develop an interpretable breast cancer risk predictor by integrating our encoder into the AsymMIRAI~\cite{donnelly2024asymmirai} framework. By replacing the original vision encoder with Mammo-CLIP's, we leverage its superior ability to detect subtle bilateral dissimilarities. Second, we propose a novel mammography report generator capable of processing all four screening views (Left-CC, Left-MLO, Right-CC, Right-MLO) simultaneously. Unlike existing single-image report generators \eg LLaVA-Med or MedGemma, our model utilizes four parallel, frozen Mammo-CLIP vision encoders. We develop the report generator in two stages using a combined dataset of 19,811 study-report pairs from Boston University and UPMC. In the first stage, we learn a projector module to align the frozen mammo-CLIP vision encoder with a large language model. In the second stage, we generated 298,285 high-quality question-answering pairs from the dataset to fine-tune both the projector and the LLM concurrently. 

To address these challenges, this paper proposes Mammo-CLIP, a vision-language model specifically designed for mammography. Unlike generalist approaches, Mammo-CLIP processes high-resolution 2D screening mammograms (1520$\times$912), preserving fine diagnostic details. To learn robust representations, we pre-train Mammo-CLIP on a multi-center corpus of 140,677 patients (821,326 screening mammograms) across 4 hospitals -- University of Pittsburgh Medical Center (UPMC), Boston University (BU), Emory Breast Imaging Dataset (EMBED), Mayo Clinic using a dual strategy of report synthesis and multi-view supervision. This dataset represents the largest and most diverse mammography pre-training corpus to date. Mammo-CLIP leverages a 30M-parameter vision encoder, which is a fraction of a 400M-parameter vision encoder in generalist models \eg MedSigLIP, therefore reducing the pre-training cost substantially. Yet, Mammo-CLIP outperforms MedSigLIP in zero-shot and data-efficient settings across core mammographic findings, including masses, calcifications, and cancer. We demonstrate the effectiveness of Mammo-CLIP on two challenging clinical applications for screening: establishing the first text-interpretable risk predictor and the first multi-view mammography report generator.

% Despite using a 30M-parameter vision encoder -- nearly a fraction of the generalist model MedSigLIP’s 400M-parameter encoder—Mammo-CLIP delivers superior zero-shot and data-efficient performance across core mammographic findings, including masses, calcifications, and cancer. W


% Mammo-CLIP achieves superior zero-shot and data-efficiency performance across core mammographic findings: \eg mass, calcification, and cancer detection. 
While MIRAI~\cite{yala2021toward} delivers strong predictive accuracy, its black-box design limits clinical trust. AsymMIRAI~\cite{donnelly2024asymmirai} introduces interpretability through bilateral dissimilarity but inherits MIRAI’s shallow ResNet-18 encoder. Critically, neither model contains a language-aligned image encoder, making text-grounded interpretability impossible. Motivated by the superior diagnostic performance of Mammo-CLIP, we integrate its high-resolution, report-aligned vision encoder into both the MIRAI and AsymMIRAI pipelines. Mammo-CLIP’s image-text alignment enables us to highlight, for the first time, the exact sentences in the paired radiology report that correspond to the visual features driving the prediction of the risk models. We train the risk models via knowledge distillation from MIRAI's risk outputs, achieving high-performance, fully transparent prediction that is robust across in-distribution (ID) and out-of-distribution (OOD) settings. Next, we introduce a mammography report generation model -- Mammography Grounded Report Generation (Mammo-GRG). 
Unlike generalist models \eg LLaVA-Med~\cite{li2023llava} or MedGemma~\cite{sellergren2025medgemma} that process a single downsampled image, Mammo-GRG leverages four parallel Mammo-CLIP vision encoders that operate on high-resolution mammograms, a critical design choice to preserve subtle diagnostic features. To generate the preliminary report, we train Mammo-GRG using a two-stage training method: (1) an alignment stage that aligns the frozen Mammo-CLIP encoders with a large language model (Llama 3.1 8B) by training a multimodal projector using 19,811 study–report pairs (from BU and UPMC) and (ii) an instruction-tuning stage that fine-tunes the large language model and multimodal projector using 359,746 mammography QA pairs. To ensure factual consistency, a final grounding stage synthesizes the final report, combining the preliminary report with the structured, zero-shot findings from Mammo-CLIP. 
We conduct a rigorous evaluation demonstrating Mammo-GRG's superior performance over generalist models in generating reports closer to the ground truth, accurately detecting mammographic findings, and preserving robustness in out-of-distribution settings. As standard NLP metrics (\eg, BLEU, ROUGE) fail to capture clinically consequential errors in radiology, such as misreported laterality or false BI-RADS scores, we adapt the GREEN~\cite{ostmeier2024green} metric for structured, mammography-specific error analysis using GPT-4o-mini as the LLM judge. In combination, Mammo-CLIP and its downstream clinical applications in risk prediction and report generation represent a transformative step toward intelligent, workflow-aware mammography, offering the potential to augment radiologist performance, minimize documentation fatigue, and enable scalable, equitable breast cancer screening worldwide.


% >>>>>  One punch missing. 1st report generator and 1st text interpretable prognosis
% >>>> no risk predictor is aligned - say this for interpretabilty and also in the risk pred section.



==> sections/introduction_v2.tex <==
In 2022, breast cancer accounted for 2.3 million new cases and 666,000 deaths globally, making it the most diagnosed cancer worldwide \cite{bray2024global}. Early detection is critical: screening from age 40 reduces breast cancer mortality by 25\% over 10 years~\cite{duffy2020effect, trentham2024collaborative}. 
However, screening mammography presents significant challenges. 
First, it exhibits substantially high recall rates (averaging 11.5\% nationally in the U.S.) and reduced sensitivity in women with dense breast tissue \cite{lehman2017national, nelson2016factors}. 
Second, overdiagnosis poses a substantial risk leading to unnecessary treatment, \eg surgery, radiation, and endocrine therapy~\cite{ryser2022estimation}.
Third, recent guidelines in the US recommend routine screening beginning at age 40, dramatically increasing the mammography volume~\cite{nicholson2024screening}.
Such sharp growth amplifies radiologist workload. Up to 44\% of their workday involves non-interpretive tasks such as documentation and communication, compounding cognitive fatigue and driving diagnostic errors \cite{glover2017quantifying, stec2018systematic, kwee2021workload}. 
These limitations highlight the need for AI systems that integrate diagnosis, prognosis, and automated report generation. Foundation models offer a natural framework: large-scale pretraining can yield robust, generalizable mammographic representations for downstream clinical tasks.
Building on this principle, this paper introduces a mammography-specific FM pretrained on the largest multi-institutional dataset to date, integrating diagnosis, risk prediction, and report generation.


Multimodal FM achieves remarkable success in computer vision by using vision-language pretraining~\cite{radford2021learning, zhang2020contrastive, huang2021gloria, wu2023medklip, wang2022medclip}, where text provides an inexpensive and scalable supervision for learning semantically rich visual representations. This paradigm aligns naturally with screening mammography. Radiology reports capture key prognostic indicators, \eg mass, microcalcifications \etc, which serve as important risk factors for breast cancer~\cite{boyd2007mammographic, kim2022microcalcifications, azam2021mammographic}. These clinical texts can bootstrap a model's reasoning of both diagnostic and prognostic features. FMs also address the challenge of scarcity of annotated data in medical imaging, where high-quality labels are expensive to obtain.
Large-scale pretraining enables FMs to achieve strong zero-shot and linear-probe performance, enabling efficient transfer to new clinical tasks and sites with minimal labels. A FM pre-trained on large, heterogeneous data further improves out-of-distribution generalization across clinical sites. Finally, image–text alignment provides a direct path to interpretability by grounding visual evidence in natural language, supporting clinical auditing and trust~\cite{varma2023villa, zhong2022regionclip}.

% Such a model can also function as a zero-shot retrieval engine to find clinically similar precedent cases. 

One potential strategy is to construct mammography vision–language models  using generalist models, \eg MedGemma~\cite{sellergren2025medgemma} or from models pre-trained on large datasets from other imaging modalities, \eg chest X-rays~\cite{huang2021gloria, wu2023medklip, wang2022medclip}. However, these methods have fundamental limitations. Generalist models often operate on low-resolution patches (MedSigLip uses $448\times448$ image resolution), failing to capture subtle, diagnostically critical features of mammogram images \eg microcalcifications. Consequently, they exhibit poor data efficiency and zero-shot performance in the high-resolution, fine-grained mammography domain. These limitations motivate a domain-specific FM guided by four core desiderata: 1) operating directly on high-resolution images; 2) handling heterogeneous clinical data with missing reports, partial labels, or incomplete views; 3) enabling a broad suite of applications, including diagnosis, interpretable risk prediction and report generation; 4) maintaining robustness to dataset shift—generalizing reliably to unseen institutions and patient demographics.


% Overview of the method [similar to Sun-In Lee [paper]
% This needs a rewrite

\begin{figure}[p]
    \centering
    % \includegraphics[height=0.8\textheight]{figures/main.pdf}
    \includegraphics[width=0.92\textwidth]{figures/main.pdf}
    \vspace{-0.8em}
    \caption{\textbf{Overview of the Mammo-CLIP foundation model and downstream applications.} \textbf{a.} Schematic of the Mammo-CLIP framework. High-resolution mammographic views (CC, MLO) and paired radiology reports are jointly used for multi-view contrastive pretraining, aligning image and text representations within a shared embedding space (see Methods). \textbf{b.} Composition of multi-institutional pretraining datasets from the Mayo Clinic, BU, UPMC, and EMBED cohorts. \textbf{c.} Composition of evaluation datasets used to benchmark diagnostic and prognostic generalization across in-distribution (ID; EMBED) and out-of-distribution (OOD; RSNA, VinDr) settings. \textbf{d.} Pathology localization by integrating the Mammo-CLIP vision encoder into a RetinaNet detector. \textbf{e.} Zero-shot classification with Mammo-CLIP. Image and text encoders map mammograms and prompts into a shared space. Similarity between embeddings enables classification without fine-tuning. \textbf{f.} Findings classification under either linear-probe or full fine-tuning settings where a linear classifier is attached to Mammo-CLIP image encoder, quantifying the quality of the learned visual representations. \textbf{g.} Interpretable risk prediction built using frozen Mammo-CLIP encoders across CC and MLO views for 1–5 year risk estimation. \textbf{h.} Automated report generation (Mammo-GRG) combining Mammo-CLIP with a Llama-3.1-8B language model to produce clinically grounded radiology reports.}  
    \label{fig:schematic}
\end{figure}


\begin{table*}[t]
\centering
\footnotesize
\begin{threeparttable}
\caption{Summary characteristics of the EMBED, UPMC, and Mayo Clinic datasets used to pre-train Mammo-CLIP. Note that the Mammo-GRG pretraining also leverages the same UPMC dataset. }
\label{tab:main_dataset_char}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{5pt}

\begin{tabularx}{\textwidth}{l l Y Y Y}
\rowcolor{nmHeader}
\textbf{\color{nmHeadTxt} Characteristic} &
\textbf{\color{nmHeadTxt} Category} &
\textbf{\color{nmHeadTxt} EMBED (N=20,381)} &
\textbf{\color{nmHeadTxt} UPMC (N=13{,}829)} &
\textbf{\color{nmHeadTxt} Mayo Clinic (N=96{,}567)} \\

\midrule

\multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{BI-RADS}} &
0 & 5{,}476 (15.4\%) & 2{,}125 (15.4\%) & \NA \\
& 1 & 10{,}822 (31.7\%) & 4{,}376 (31.7\%) & \NA \\
& 2 & 4{,}083 (52.9\%) & 7{,}328 (52.9\%) & \NA \\
\addlinespace[3pt]\midrule

\multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Age Group}} &
$<$ 50 years & 956 (9.6\%) & 1{,}326 (9.6\%) & 2{,}476 (2.4\%) \\
& 50–60 years & 11{,}163 (44.6\%) & 6{,}163 (44.6\%) & 45{,}513 (47.3\%) \\
& $>$ 60 years & 8{,}262 (45.8\%) & 6{,}340 (45.8\%) & 48{,}578 (50.4\%) \\
\addlinespace[3pt]\midrule

\multirowcell{4}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Breast Density}} &
Almost entirely fatty (A) & 3{,}113 (22.5\%) & 6{,}159 (22.5\%) & 9{,}712 (10.0\%) \\
& Scattered fibroglandular (B) & 5{,}712 (41.3\%) & 5{,}233 (41.3\%) & 47{,}370 (49.0\%) \\
& Heterogeneously dense (C) & 3{,}801 (27.5\%) & 6{,}765 (27.5\%) & 34{,}861 (36.1\%) \\
& Extremely dense (D) & 1{,}203 (8.7\%) & 2{,}224 (8.7\%) & 4{,}624 (4.9\%) \\
\addlinespace[3pt]\midrule

\multirowcell{4}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Race}} &
Black & 8{,}580 (42.1\%) & \NA & 893 (0.9\%) \\
& White & 8{,}193 (40.2\%) & \NA & 92{,}287 (95.3\%) \\
& Asian & 1{,}305 (6.4\%) & \NA & 1{,}713 (1.7\%) \\
& Other & 2{,}303 (11.3\%) & \NA & 1{,}674 (1.7\%) \\
\addlinespace[3pt]\midrule

\multirowcell{5}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Manufacturer}} &
HOLOGIC, Inc. & \NA & 13{,}443 (96.7\%) & 90{,}351 (93.5\%) \\
& LORAD & \NA & 287 (2.1\%) & 1{,}359 (1.5\%) \\
& SIEMENS & \NA & 99 (0.7\%) & 5 ($<$0.1\%) \\
& Visage & \NA & \NA & 20 ($<$0.1\%) \\
& Unknown & \NA & \NA & 4{,}832 (5.0\%) \\

\bottomrule
\end{tabularx}

\begin{tablenotes}[flushleft]\footnotesize
\item \textbf{Note:} Missing entries are indicated by \NA. BI-RADS categories follow standard clinical grading; percentages are computed relative to total patient count.
\end{tablenotes}
\end{threeparttable}
\end{table*}


\begin{table*}[t]
\centering
\footnotesize
\begin{threeparttable}
\caption{Characteristics of BU datasets. It consists of 54,776 screening images from 9,900 patients and 13,480 exams with complete data, that includes an associated radiology report and followup data on clinical outcomes. It is one of the pretraining datasets used to pre-train Mammo-CLIP and Mammo-GRG. Among the 1,041 total cancer cases, the number of cases occurring within years 1–5 are 283, 212, 205, 188, and 153, respectively.}
\label{tab:bu_dataset_characteristics}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{5pt}

\begin{tabularx}{\textwidth}{l l Y Y}
\rowcolor{nmHeader}
\textbf{\color{nmHeadTxt} Characteristic} &
\textbf{\color{nmHeadTxt} Category} &
\textbf{\color{nmHeadTxt} All} &
\textbf{\color{nmHeadTxt} Cases} \\
\midrule

\rowcolor{nmSubhdr}\textbf{Exams} &  & 13{,}480 & 1{,}041 \\
\addlinespace[3pt]\midrule

\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Age at screening}} &
Median (y) & 56 & 62 \\
& Range (y) & 24--87 & 34--87 \\
\addlinespace[3pt]\midrule

\multirowcell{3}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Age groups}} &
$<$ 50 y & 3{,}878 (28.7\%) & 114 (10.9\%) \\
& 50--70 y & 7{,}990 (59.3\%) & 747 (71.8\%) \\
& $>$ 70 y & 1{,}617 (12.0\%) & 180 (17.3\%) \\
\addlinespace[3pt]\midrule

\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Family history of breast cancer.}} &
 No & 12{,}950 (96.1\%) & 930 (89.3\%) \\
& Yes & 530 (3.9\%) & 111 (10.7\%) \\
\addlinespace[3pt]\midrule

\multirowcell{2}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{History of breast biopsy}} &
 No prior biopsy & 12{,}901 (95.7\%) & 922 (88.6\%) \\
& Prior biopsy, benign dx unknown & 579 (4.3\%) & 119 (11.4\%) \\
\addlinespace[3pt]\midrule

\multirowcell{5}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Mammographic density}} &
 Almost entirely fatty (A) & 3{,}428 (25.4\%) & 190 (18.3\%) \\
& Scattered fibroglandular (B) & 4{,}792 (35.6\%) & 524 (50.3\%) \\
& Heterogeneously dense (C) & 3{,}824 (28.3\%) & 268 (25.7\%) \\
& Extremely dense (D) & 1{,}323 (9.8\%) & 50 (4.8\%) \\
& Unknown & 113 (0.8\%) & 9 (0.9\%) \\
\addlinespace[3pt]\midrule

\multirowcell{4}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{BI-RADS}} &
 0 & 1{,}333 (9.9\%) & 319 (30.6\%) \\
& 1 & 11{,}062 (82.1\%) & 620 (59.6\%) \\
& 2 & 1{,}053 (7.8\%) & 81 (7.8\%) \\
& Other & 32 (0.2\%) & 21 (2.0\%) \\
\addlinespace[3pt]\midrule

% \multirowcell{5}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Final BI-RADS}} &
%  1 & 11{,}479 (85.1\%) & 637 (61.2\%) \\
% & 2 & 1{,}308 (9.7\%) & 112 (10.8\%) \\
% & 3 & 341 (2.6\%) & 26 (2.5\%) \\
% & 4--5 & 294 (2.2\%) & 189 (18.1\%) \\
% & Other & 58 (0.4\%) & 53 (5.1\%) \\
% \addlinespace[3pt]\midrule

\multirowcell{6}[-.2ex][l]{\cellcolor{nmSubhdr}\textbf{Race and ethnicity}} &
 Black & 7{,}224 (53.6\%) & 557 (53.5\%) \\
& White & 2{,}573 (19.1\%) & 185 (17.8\%) \\
& Hispanic & 3{,}219 (23.9\%) & 251 (24.1\%) \\
& Asian & 327 (2.4\%) & 31 (3.0\%) \\
& Native American & 31 (0.2\%) & 3 (0.3\%) \\
& Unknown & 106 (0.8\%) & 14 (1.3\%) \\

\bottomrule
\end{tabularx}

\begin{tablenotes}[flushleft]\footnotesize
\item \textbf{Note:} Percentages are relative to the row’s population (\textbf{All} or \textbf{Cases}). Cases denotes \textbf{cancer cases}. Abbreviations: dx, diagnosis. Family history of breast cancer denotes cancer in first-degree relative(s).
\end{tablenotes}
\end{threeparttable}
\end{table*}



To address these challenges, this paper proposes Mammo-CLIP, a vision-language model specifically designed for mammography. Mammo-CLIP leverages dual image (EfficientNet-B5) and text (ModernBERT finetuned with $\sim200k$ chest CT reports) encoders to jointly process mammograms and their paired reports, optimizing a multiview contrastive loss that aligns both modalities within a shared embedding space (Methods and Fig.~\ref{fig:schematic}a). Unlike generalist FMs, Mammo-CLIP processes high-resolution 2D screening mammograms (1520$\times$912), preserving fine diagnostic details. To learn robust representations, we pre-train Mammo-CLIP on a multi-center corpus of 140,677 patients (821,326 screening mammograms) across 4 US hospitals -- University of Pittsburgh Medical Center or UPMC (13,829 patients; 46,433 screening mammograms), Boston University or BU (9,900 patients; 54,776 screening mammograms), Emory Breast Imaging Dataset or EMBED (20,381 patients; 255,039 screening mammograms), Mayo Clinic (96,567 patients; 465,078 screening mammograms) (refer to Tab.~\ref{tab:main_dataset_char} and Tab.~\ref{tab:bu_dataset_characteristics}). This dataset represents the largest and most diverse mammography pre-training corpus to date. 
Despite using a 30M-parameter vision encoder -- compared with the 400M-parameter MedSigLIP encoder in MedGemma -- Mammo-CLIP outperforms MedSigLIP in zero-shot and data-efficient settings across public in-distribution (ID) and out-of-distribution (OOD) benchmarks, all at a fraction of the pretraining cost. 
We demonstrate the effectiveness of Mammo-CLIP on two challenging clinical applications: the first text-interpretable risk predictor and the first multi-view mammography report generator.
Current risk prediction models such as MIRAI~\cite{yala2021toward} and AsymMIRAI~\cite{donnelly2024asymmirai} lack language-aligned encoders, making text-grounded interpretability impossible.
Motivated by the superior diagnostic performance of Mammo-CLIP, we integrate its high-resolution, report-aligned vision encoder into both the MIRAI and AsymMIRAI pipelines.
Mammo-CLIP’s image-text alignment enables us to highlight the specific sentences in the paired radiology report that correspond to the visual features driving the prediction of the risk models. 
Along with the interpretability, Mammo-CLIP-based risk predictors achieve high performance across ID and public OOD datasets. We then introduce Mammo-GRG, a high-resolution, multi-view mammography report generator.
Unlike generalist models \eg LLaVA-Med~\cite{li2023llava} or MedGemma~\cite{sellergren2025medgemma} that process a single downsampled image, Mammo-GRG leverages four parallel Mammo-CLIP vision encoders, thus operating on high-resolution mammograms. A two-stage training approach -- (1) alignment of frozen encoders with an LLM (Llama 3.1 8B) using 19,811 study–report pairs, and (2) instruction tuning with 359,746 mammography QA pairs -- generates the prilimninary report. A final grounding stage combines the preliminary text with zero-shot Mammo-CLIP findings to synthesize a factually consistent final report. As standard NLP metrics (\eg, BLEU) fail to capture clinically consequential errors in radiology, such as misreported laterality or false BI-RADS scores, we adapt the GREEN~\cite{ostmeier2024green} metric for structured, mammography-specific evaluation using GPT-4o-mini as the LLM judge. Mammo-GRG outperforms generalist models in report fidelity, finding-level accuracy, and OOD robustness. Together, Mammo-CLIP and its downstream applications advance mammography AI toward high-resolution, interpretable, and clinically reliable workflows.

==> sections/prognosis_v1.tex <==
% * why do we need this experiment
% * experimental setup
% * baselines
% * metric
% * dataset
% * important result


Accurate, interpretable breast cancer risk prediction is critical for tailoring screening strategies to save lives through early detection. The current state-of-the-art deep learning model, MIRAI~\cite{yala2021toward}, demonstrates high predictive accuracy but operates as a ``black box.''
MIRAI aggregates the latent representations from all four mammogram views using a transformer, limiting interpretability. This lack of transparency prevents clinical auditing and poses a significant barrier to trust and safe integration. The recent AsymMIRAI~\cite{donnelly2024asymmirai} model successfully addresses this limitation. It demonstrates that MIRAI’s performance stems primarily from bilateral dissimilarity. Motivated by this principle, AsymMIRAI aims for an interpretable model that generates heat maps to explain its predictions. However, AsymMIRAI is still constrained by the original, relatively small ResNet-18 vision encoder from MIRAI. We hypothesize that a more powerful, domain-specific vision encoder can yield a model that is both highly accurate and fully interpretable. To overcome these limitations, we develop an interpretable risk predictor on the foundation of our Mammo-CLIP (Multi-institution) model. Its powerful EfficientNet-B5 vision encoder is designed to process high-resolution mammograms, preserving the subtle pathological features that are critical for breast cancer risk assessment. In addition, the model’s joint vision–language representation enables direct alignment between image features and clinically meaningful textual concepts, supporting interpretable, language-grounded risk reasoning. 

% , whose powerful EfficientNet-B5 vision encoder, pre-trained with rich image-text representations, is poised to capture more nuanced risk signals. Furthermore, Mammo-CLIP's innate alignment with a text encoder creates a pathway for more sophisticated, text-based interpretability.

\begin{figure}[p]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/prognosis.pdf}
    \caption{\textbf{Integrating Mammo-CLIP representations with risk prediction pipelines and interpretable modeling.} \textbf{a-c.} We replace the standard ResNet-18 encoder in MIRAI and AsymMIRAI with a Mammo-CLIP-trained encoder that aligns images and reports, enabling richer and more transferable representations.
    \textbf{b.} We train two new risk predictors: MIRAI w/ Mammo-CLIP and AsymMIRAI w/ Mammo-CLIP using knowledge distillation from the original MIRAI model, preserving calibrated 1–5-year risk outputs. \textbf{d.} The Matryoshka Sparse Autoencoder (SAE) trains on 2048-dimensional spatial Mammo-CLIP features (48×29 patch grid) and expands them into a 16,384-dimensional sparse latent space, creating interpretable neuron-level representations. \textbf{e.} Risk predictors use SAE features for interpretability: turning neurons on and off quantifies their effect on risk. Shapley analysis ranks neurons by their contribution, linking top activations to both spatial image regions and key radiology report sentences.
    \textbf{f.} Comparison of AUROC for 1–5-year risk prediction  MIRAI w/ Mammo-CLIP, AsymMIRAI w/ Mammo-CLIP, and their baselines, showing that Mammo-CLIP-based encoders improve performance while maintaining interpretability. 
    \textbf{g.} Correlation between MIRAI and MIRAI w/ Mammo-CLIP risks demonstrates consistent risks across 5-year time horizons.
    \textbf{h.} SAE-reconstructed features retain discriminative fidelity in classification and detection relative to original Mammo-CLIP features.
    \textbf{i.} Qualitative visualization of MIRAI w/ Mammo-CLIP risk interpretation for high-risk 1-year cases. The top example highlights a neuron selective for mass features (MIRAI risk = 0.07), and the bottom highlights a calcification-selective neuron (MIRAI risk = 0.15). In both cases, radiology reports confirm the corresponding findings, underscoring the alignment between learned neuron activations and clinical evidence.
    }  
    \label{fig:prognosis}
\end{figure}

Our risk predictor adopts the interpretable AsymMIRAI framework (Fig.~\ref{fig:prognosis}a and Methods). The model processes the four standard views (LCC, RMLO, \etc) of screening mammograms as input. Each view passes through a dedicated, frozen Mammo-CLIP vision encoder, which extracts high-resolution feature representations. Subsequent layers compute a localized bilateral dissimilarity score for the CC and MLO view pairs. For each pair, the model identifies a ``prediction window'' corresponding to the maximum dissimilarity. The final risk score is the average of these two maximum scores. Training the risk predictor follows a knowledge distillation~\cite{hinton2015distilling} strategy on the Boston University (BU) dataset. With the Mammo-CLIP encoders kept frozen, we only optimize the dissimilarity-computing layers to approximate the 5-year risk predictions produced by MIRAI. We evaluate the model's performance using the Area Under the Receiver Operating Characteristic (AUROC) curve, with MIRAI and AsymMIRAI serving as baselines. For in-distribution (ID) evaluation on the BU dataset, we evaluate the performance of 1- to 5-year risk prediction. To assess generalization, we conduct an out-of-distribution (OOD) evaluation on the RSNA dataset. For this OOD task, the model's 1-year risk score is used to predict cancer labels, as this short-term horizon serves as a strong proxy for detecting existing cancer cases.

Fig.~\ref{fig:prognosis}b illustrates that our Mammo-CLIP-based risk predictor consistently and substantially outperforms the interpretable AsymMIRAI baseline across all prediction horizons for the ID evaluation on the Boston University dataset. For 1-year risk prediction, our model achieves an AUROC of 0.79, marking a 25\% improvement over AsymMIRAI (AUROC = 0.63). This strong performance is sustained across longer time horizons, with our model showing a 14\% improvement at the 5-year mark (AUROC = 0.67 vs. 0.59). While the black-box MIRAI model sets the highest benchmark (AUROC = 0.87 for year 1), our interpretable model successfully closes over 67\% of the performance gap between AsymMIRAI and MIRAI for 1-year risk. Fig.~\ref{fig:prognosis}d demonstrates that our Mammo-CLIP-based risk predictor demonstrates robust performance, achieving an AUROC of 0.67 on the OOD RSNA dataset. This marks a 17.5\% improvement over the interpretable AsymMIRAI baseline, whose performance degrades significantly to an AUROC of 0.57 in this challenging setting. While the black-box MIRAI model achieves an AUROC of 0.84, our model successfully closes over 37\% of the performance gap between AsymMIRAI and MIRAI. This result highlights the superior generalization of the features learned by the Mammo-CLIP encoder, confirming its ability to maintain predictive power in new, unseen clinical environments. Fig.~\ref{fig:prognosis}c and~\ref{fig:prognosis}d (bottom panel) report the qualitative examples to visualize our model's high-risk prediction for a patient for ID (BU) and OOD (RSNA) settings, respectively. The model exhibits remarkable location consistency, as the prediction window remains stable on the same tissue region each year, providing a transparent basis for its high-risk assessment.

==> sections/prognosis_v2.tex <==
% * why do we need this experiment
% * experimental setup
% * baselines
% * metric
% * dataset
% * important result

% * why do we need this experiment
% Accurate, interpretable breast cancer risk prediction is critical for tailoring screening strategies to save lives through early detection. The current state-of-the-art deep learning model, MIRAI~\cite{yala2021toward}, demonstrates high predictive accuracy but operates as a ``black box.''
% MIRAI aggregates the latent representations from all four mammogram views using a transformer, limiting interpretability. This lack of transparency prevents clinical auditing and poses a significant barrier to trust and safe integration. The recent AsymMIRAI~\cite{donnelly2024asymmirai} model successfully addresses this limitation. It demonstrates that MIRAI’s performance stems primarily from bilateral dissimilarity. Motivated by this principle, AsymMIRAI aims for an interpretable model that generates heat maps to explain its predictions. However, AsymMIRAI is still constrained by the original, relatively small ResNet-18 vision encoder from MIRAI (Fig.~\ref{fig:prognosis}a). We hypothesize that a more powerful, domain-specific vision encoder can yield a model that is both highly accurate and fully interpretable. We take it to next level by attaching mammo-clip (Multi-institution) image encoder. Its powerful mammogram-report-aligned EfficientNet-B5 vision encoder is designed to process high-resolution mammograms, preserving the subtle pathological features that are critical for breast cancer risk assessment. In addition, the model’s joint vision–language representation enables direct alignment between image features and clinically meaningful textual concepts, supporting interpretable, language-grounded risk reasoning. 
% Bold statement: AsymMIRAI and MIRAI can not do textual interpretability bcz their image encoder is not language aligned

% % % * experimental setup
% Two risk predictor - attach to mirai (Fig.~\ref{fig:prognosis}b) -- MIRAI w/ Mammo-CLIP and attach to asymirai (Fig.~\ref{fig:prognosis}c) -- AsymMIRAI w/ Mammo-CLIP
% MIRAI w/ Mammo-CLIP trained on KD loss from MIRAI 1-5 yr risk and spits 1-5 yr risk.
% AsymMIRAI w/ Mammo-CLIP trained on KD loss from 5 yr risk from MIRAI and spits risk score.
% Training the risk predictor follows a knowledge distillation~\cite{hinton2015distilling} strategy on the Boston University (BU) dataset.

% MIRAI w/ Mammo-CLIP - The model processes the four standard views (LCC, RMLO, \etc) of screening mammograms as input. Each view passes through a dedicated, frozen Mammo-CLIP vision encoder, which extracts high-resolution feature representations. feautures from MIRAI go to the transformer layer which is image aggregator. The architecture of transformer is same as MIRAI. Then mean pool image representations followed by linear classifier to predict 1-5 yr risks.
% the Mammo-CLIP encoders kept frozen. For AsymMIRAI, we only optimize the dissimilarity-computing layers to approximate the 5-year risk predictions produced by MIRAI.

% AsymMIRAI w/ Mammo-CLIP --
% The model processes the four standard views (LCC, RMLO, \etc) of screening mammograms as input. Each view passes through a dedicated, frozen Mammo-CLIP vision encoder, which extracts high-resolution feature representations. Subsequent layers compute a localized bilateral dissimilarity score for the CC and MLO view pairs. For each pair, the model identifies a ``prediction window'' corresponding to the maximum dissimilarity. The final risk score is the average of these two maximum scores.


% We evaluate the model's performance using the Area Under the Receiver Operating Characteristic (AUROC) curve, with MIRAI and AsymMIRAI serving as baselines. For in-distribution (ID) evaluation on the BU dataset, we evaluate the performance of 1- to 5-year risk prediction. To assess generalization, we conduct an out-of-distribution (OOD) evaluation on the RSNA dataset and VinDr. For this OOD task, the model's 1-year risk score is used to predict cancer labels, as this short-term horizon serves as a strong proxy for detecting existing cancer cases.

% For interpretability, train Matryoshka Sparse Autoencoder (MSAE) (Fig.~\ref{fig:prognosis}d) — an interpretable neural architecture trained on Mammo-CLIP features to predict breast cancer risk while preserving clinical explainability. using BU dataset. Each image is encoded with Mammo-CLIP, yielding 2048-dimensional spatial features (48×29 grid of patches). Expands to a 16,384-dim latent space, enforcing different sparsity levels (16 384 active neurons).

% Shapley value (Fig.~\ref{fig:prognosis}d) computation for finding neurons highly predictive of risk: Calculating the value for every possible combination of 16,384 neurons is computationally impossible (it's $2^{16384}$ combinations).So, the researchers use a "Monte Carlo approximation". Instead of testing all combinations, they test a large number of random combinations (samples) to get a very good estimate. (get this part from the uploaded paper.content1.pdf attached) After calculating the Shapley value for all 16,384 neurons, the researchers can rank them by their contribution to the risk score.



Accurate, interpretable breast cancer risk prediction is critical for tailoring screening strategies to save lives through early detection. The current state-of-the-art deep learning model, MIRAI~\cite{yala2021toward}, demonstrates high predictive accuracy but operates as a ``black box.''
MIRAI aggregates the latent representations from all four mammogram views using a transformer, limiting interpretability. This lack of transparency prevents clinical auditing and poses a significant barrier to trust and safe integration. The recent AsymMIRAI~\cite{donnelly2024asymmirai} model successfully addresses this limitation. It demonstrates that MIRAI’s performance stems primarily from bilateral dissimilarity. Motivated by this principle, AsymMIRAI aims for an interpretable model that generates heat maps to explain its predictions. However, AsymMIRAI is still constrained by the original, relatively small ResNet-18 vision encoder from MIRAI. Moreover, neither MIRAI nor AsymMIRAI can provide textual interpretability because their encoders are not aligned with radiology reports. Mammo-CLIP (multi-institution) resolves this limitation by jointly training on paired mammograms and radiology reports across multiple institutions. Its vision encoder, an EfficientNet-B5 architecture optimized for high-resolution mammograms, learns image representations that are intrinsically aligned with clinical language. This alignment enables two complementary interpretability axes -- image-based and text-based—that are grounded in the same semantic space.

We integrate the frozen Mammo-CLIP (multi-institution) encoder into both MIRAI and AsymMIRAI pipelines (Fig.~\ref{fig:prognosis}a-b), producing MIRAI w/ Mammo-CLIP and AsymMIRAI w/ Mammo-CLIP. Both utilize individual encoders for the four standard mammographic views (LCC, LMLO, RCC, RMLO) to extract view-specific representations. MIRAI w/ Mammo-CLIP leverages a transformer aggregator, followed by a mean pooling layer and a linear classifier to predict 1–5 year risks. Alternatively, AsymMIRAI w/ Mammo-CLIP uses Mammo-CLIP-extracted view-specific representation to compute a localized bilateral dissimilarity score. The final risk score is the average of the two maximum-dissimilarity regions, identifying the most anomalous tissue. We optimize both risk predictors using the knowledge distillation loss from the original MIRAI model (see Methods and Fig~\ref{fig:app_prognosis}). 

To move beyond simple heatmaps and achieve multimodal interpretability, we first train a Matryoshka Sparse Autoencoder (SAE)~\cite{zaigrajew2025interpreting} on Mammo-CLIP's 2048-dimensional image representations (Fig.~\ref{fig:prognosis}c). Motivated from~\cite{nakka2025mammo}, the SAE expands these features into a 16,384-dimensional sparse latent space, effectively creating an interpretable, neuron-level ``vocabulary'' for mammographic features, \eg mass, calcification. We apply Shapley value analysis~\cite{lundberg2017unified} (Fig.~\ref{fig:prognosis}d) to quantify each neuron’s causal influence on the predicted risk. Exact computation across all 16,384 neurons is infeasible, so we adopt a permutation-based Monte Carlo approximation. In each iteration, the algorithm samples a random permutation of all neurons and measures a target neuron’s marginal contribution by comparing the model’s risk score with and without that neuron, given all neurons preceding it in the permutation. Averaging these marginal effects over 100 random samples yields an unbiased estimate of the neuron’s Shapley value, capturing its direct causal impact on the model’s risk prediction. We identify risk-increasing neurons—those with positive Shapley values—and rank them by magnitude. For each high-ranking neuron, we generate a spatial activation heatmap that localizes the mammographic regions driving the predicted risk.
Unlike existing risk predictors such as MIRAI and AsymMIRAI, which rely solely on image encoders without language grounding, our framework provides text-level interpretability by leveraging Mammo-CLIP’s contrastive image–text alignment. For each high-risk neuron, we perform causal ablation by suppressing its activation and generating a reconstructed, ``ablated'' image representation. We then compute the similarity between this ablated feature and every sentence in the paired radiology report. The sentence that exhibits the largest drop in similarity serves as the neuron’s semantic identifier. This mechanism directly links the model’s visual reasoning to clinically meaningful language, connecting a risk-driving visual concept (\eg a mass-selective neuron) to its corresponding textual descriptor (\eg  ``a suspicious mass is seen'').


\begin{figure}[p]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/prognosis.pdf}
    \caption{\textbf{Integrating Mammo-CLIP representations with risk prediction pipelines and interpretable modeling.} \textbf{a.} Training pipeline of the risk predictors -- MIRAI w/ Mammo-CLIP and AsymMIRAI w/ Mammo-CLIP using knowledge distillation from 1–5-year risk outputs of the original MIRAI model. We freeze the image encoder throughout the training.
    \textbf{b.} We replace the standard ResNet-18 encoder in MIRAI and AsymMIRAI with a Mammo-CLIP-trained encoder that aligns images and reports, enabling richer and more transferable representations.
    \textbf{c.} The Matryoshka Sparse Autoencoder (SAE) trains on 2048-dimensional spatial Mammo-CLIP features (48×29 patch grid) and expands them into a 16,384-dimensional sparse latent space, creating interpretable neuron-level representations. 
    \textbf{d.} Risk predictors use SAE features for interpretability: turning neurons on and off quantifies their effect on risk. Shapley analysis ranks neurons by their contribution, linking top activations to both spatial image regions and key radiology report sentences.
    \textbf{e.} Comparison of AUROC for cancer prediction  MIRAI w/ Mammo-CLIP, AsymMIRAI w/ Mammo-CLIP, and their baselines for VinDr (OOD) and RSNA (OOD) datasets. Each curve reports the mean AUROC with 95\% confidence intervals (CIs).
    \textbf{f.} Comparison of AUROC for 1–5-year risk prediction  MIRAI w/ Mammo-CLIP, AsymMIRAI w/ Mammo-CLIP, and their baselines using BU (ID) dataset, showing that Mammo-CLIP-based encoders improve performance while maintaining interpretability. Each curve reports the mean AUROC with 95\% confidence intervals (CIs).
    \textbf{g.} Correlation between MIRAI and MIRAI w/ Mammo-CLIP risks demonstrates consistent risks across 5-year time horizons using BU (ID) dataset. Reported correlation coefficients (Pearson’s $r$) with 95\% CIs.
     \textbf{h.} SAE-reconstructed features retain discriminative fidelity in classification and detection relative to original Mammo-CLIP features.
    \textbf{i.} Qualitative visualization of MIRAI w/ Mammo-CLIP risk interpretation for a high-risk 1-year case (MIRAI risk = 0.74) in the BU dataset shows dual interpretability: image-based saliency highlights a neuron selective for mass features, while the corresponding report sentence yields the highest similarity drop for risk, indicating language-based interpretability. 
    }  
    \label{fig:prognosis}
\end{figure}

We evaluate each risk predictor's performance using the Area Under the Receiver Operating Characteristic (AUROC) curve, with MIRAI and AsymMIRAI serving as baselines. We train MIRAI w/ Mammo-CLIP and AsymMIRAI w/ Mammo-CLIP with the BU data (same training split used to train Mammo-CLIP). For in-distribution (ID) evaluation on the BU dataset, we evaluate the performance of 1- to 5-year risk prediction. To evaluate generalization, we conduct an out-of-distribution (OOD) evaluation on the RSNA dataset and VinDr. For this OOD task, the model's 1-year risk score is used to predict cancer labels, as this short-term horizon serves as a strong proxy for detecting existing cancer cases.

Fig~\ref{fig:prognosis} e-f compares the performance of different risk models for the OOD (VinDr and RSNA) and ID (BU) datasets, respectively. Across all evaluation years, AsymMIRAI w/ Mammo-CLIP shows a marked improvement over the original AsymMIRAI, increasing AUROC by $\sim$26–36\% (\eg, for year 1: 0.79 vs. 0.63). While the black-box MIRAI model establishes the highest benchmark (AUROC = 0.87, 95\% CI: 0.81–0.92), MIRAI w/ Mammo-CLIP achieves a comparable performance (AUROC = 0.85, 95\% CI: 0.79–0.91), indicating that the multimodal encoder retains MIRAI’s predictive strength while enhancing interpretability. Across both VinDr and RSNA OOD datasets, AsymMIRAI w/ Mammo-CLIP outperforms the original AsymMIRAI (VinDr: AUROC = 0.70 \vs 0.60; RSNA: 0.67 \vs 0.57), representing a relative gain of 15–18\%. MIRAI w/ Mammo-CLIP achieves an AUROC of 0.80 (VinDr) and 0.79 (RSNA), remaining within 3–4\% of the original MIRAI (0.83 and 0.80, respectively). Fig~\ref{fig:prognosis} h compares the discriminative performance of the original Mammo-CLIP features and the Matryoshka Sparse Autoencoder (MSAE)–reconstructed features across classification (AUROC) and detection (mAP) tasks. The reconstructed features preserve nearly identical performance to the original representations (\eg Mass: AUROC 0.77 \vs 0.79; Calcification: 0.95 \vs 0.95; Detection mAP differences $\leq0.04$), indicating minimal information loss. The preserved fidelity of the reconstructed features enables their use for neuron-level interpretability across image and text modalities. Fig.~\ref{fig:prognosis}i illustrates qualitative interpretability of the MIRAI w/ Mammo-CLIP risk predictor for a high-risk 1-year case (MIRAI risk: 0.74). The saliency heatmap highlights the spatial activation of the highest-contributing neuron identified by Shapley analysis, localizing to a mass region in the left breast. The corresponding radiology report sentence (``Mass in the left breast needs additional imaging'') exhibits the largest drop in image–text similarity after neuron ablation, confirming that the neuron encodes a clinically meaningful finding (refer to Fig~\ref{fig:app_text_interpretability} for more examples).



% Fig.~\ref{fig:prognosis}d demonstrates that our Mammo-CLIP-based risk predictor demonstrates robust performance, achieving an AUROC of 0.67 on the OOD RSNA dataset. This marks a 17.5\% improvement over the interpretable AsymMIRAI baseline, whose performance degrades significantly to an AUROC of 0.57 in this challenging setting. While the black-box MIRAI model achieves an AUROC of 0.84, our model successfully closes over 37\% of the performance gap between AsymMIRAI and MIRAI. This result highlights the superior generalization of the features learned by the Mammo-CLIP encoder, confirming its ability to maintain predictive power in new, unseen clinical environments. Fig.~\ref{fig:prognosis}c and~\ref{fig:prognosis}d (bottom panel) report the qualitative examples to visualize our model's high-risk prediction for a patient for ID (BU) and OOD (RSNA) settings, respectively. The model exhibits remarkable location consistency, as the prediction window remains stable on the same tissue region each year, providing a transparent basis for its high-risk assessment.

==> sections/report_generation_v1.tex <==
Observing Mammo-CLIP's superior performance, we develop the first multi-view Mammography Grounded Report Generator (Mammo-GRG) for screening mammography. Our report generator integrates the pre-trained Mammo-CLIP (multi-institution) vision encoder, a multimodal projector, and a Llama 3.1 8B large language model (LLM)~\cite{grattafiori2024llama}. We use the same multimodal projector design as CT-CHAT~\cite{hamamci2024developing}. To effectively align the visual and language modalities, we employ a two-stage training method~\cite{liu2023visual, hamamci2024developing}. First, we conduct a vision-language alignment stage to align the vision encoder with the LLM. In this stage, with both the vision encoder and LLM frozen, we train only the multimodal projector to predict the full radiology report from the image representations. Next, we perform an end-to-end instruction tuning stage, where we fine-tune both the projector and the LLM on a dataset of 359,746 question-answer (QA) pairs (refer to Fig.~\ref{fig:app_mammo_instruct} for the QA distributions) derived from Boston University and UPMC radiology reports. Refer to Tab.~\ref{tab:prompt_mammo_instruct} and~\ref{tab:prompt_multitype} for the corresponding prompts to generate the QA pairs from GPT4o. Mammo-GRG overcomes three core challenges: multi-view image integration, data imbalance, and clinical grounding of generated text (Fig.~\ref{fig:report_generator}a and Methods).

First, to handle the four distinct views of a screening mammogram (LCC, LMLO, RCC, RMLO), Mammo-GRG extracts image representations for each view through a dedicated, parallel Mammo-CLIP vision encoder (multi-institution). Next, we encapsulate the extracted image representations within view-specific tokens (\texttt{\textless LCC\textgreater, \textless LMLO\textgreater, \textless RCC\textgreater, \textless RMLO\textgreater}) that explicitly encode view identity for the LLM. Next, a multimodal projector projects each view representation into the LLM’s latent space. Following the projection, we add a learned per-view positional embedding to each token to preserve spatial and semantic distinctions among the four standard views. This positional embedding enables Mammo-GRG to maintain cross-view consistency and prevents information leakage between left–right or CC–MLO representations, which is essential for accurate reasoning about asymmetric findings.  Second, to mitigate data imbalance across clinical cohorts, we parse the BU and UPMC reports using GPT-4o to create structured labels for mass, calcification, architectural distortion, and asymmetry. We select these findings as they represent the most common and clinically significant indicators of breast cancer in screening populations, whereas other findings occur too infrequently in the dataset to support robust modeling. From these structured labels, we assign each examination a binary indicator for the presence of a specific mammographic finding. Specifically, an exam is marked positive if at least one of the four findings is present. We track the counts of positive and negative cases to compute inverse-frequency sampling weights, ensuring balanced representation of both groups during training. Refer to Tab.~\ref{tab:mammo_grg_system_prompt} for the system prompt to generate the preliminary report using Llama 3.1 8B.
Third, to ensure the clinical fidelity of the generated reports, Mammo-GRG integrates a grounding step in which Mammo-CLIP (refer to Tab.~\ref{tab:mammo_grg_grounding_prompt} for the corresponding prompt), operating in a zero-shot mode, predicts the presence of key mammographic findings directly from the input mammograms. The resulting structured outputs constrain the report generation process, ensuring that textual descriptions remain consistent with image-derived evidence.

% Second, to mitigate data imbalance across clinical cohorts, we parse the BU and UPMC reports using GPT-4o to create structured labels for mass, calcification, architectural distortion, and asymmetry. We then derive a case-level, binary indicator of finding presence, defined as positive if an exam contained at least one of these specified findings, which we use for balanced dataset sampling during training.

% This embedding functions as a view identifier, analogous to segment embeddings in NLP, conditioning the model to process features in a view-aware manner.
% Critically, to ensure the Mammo-GRG disambiguates visual tokens from different views, we augment each view’s projected queries with a learned, per-view positional embedding.
\begin{figure}[p]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/report_generator.pdf}
    \vspace{-0.8em}
    \caption{\textbf{Overview of Mammo-GRG}. \textbf{a.} Schematic of the Mammo-GRG architecture. Four-view screening mammograms (LCC, LMLO, RCC, RMLO) are encoded by dedicated Mammo-CLIP vision encoders and projected to the latent space of a Llama-3.1-8B language model via a multimodal projector. View-specific tokens and positional embeddings preserve spatial and semantic distinctions, enabling cross-view reasoning. \textbf{b.} Clinical grounding stage where Mammo-GRG generates the final radiology report from the preliminary report. Mammo-GRG leverages Mammo-CLIP in zero-shot mode to predict key findings (mass, calcification, asymmetry) that constrain report generation. \textbf{c.} The GREEN evaluation framework evaluates the factual and clinical correctness of the generated report by comparing candidate and target reports using an LLM judge (GPT-4o-mini). \textbf{d.} Structured findings are extracted from both generated and reference reports using GPT-4o-mini. \textbf{e–f} Lexical (BLEU-1, ROUGE-L) and clinical (GREEN) performance on BU and UPMC datasets demonstrate consistent improvements of Mammo-GRG over fine-tuned MedGemma and LLaVA-Med baselines. \textbf{g.} Recall of key mammographic findings extracted from generated versus reference reports across datasets and laterality, showing higher clinical recall for Mammo-GRG. \textbf{h.} Pathological grounding evaluation, showing recall for mass and calcification findings extracted from generated reports compared directly to image-level ground-truth labels on the in-distribution (EMBED) and out-of-distribution (VinDr) datasets. Mammo-GRG maintains strong predictive alignment with actual imaging findings. \textbf{i.} Qualitative example illustrating the GREEN score assessment of a Mammo-GRG-generated report against ground truth, highlighting accurate recovery of findings and clinical consistency.}   
    \label{fig:report_generator}
\end{figure}

%  GREEN decompose - write about green
We conduct a comprehensive and rigorous evaluation of report-generation performance across lexical, clinical, and pathological axes. For lexical assessment, BLEU-1 and ROUGE-L quantify linguistic overlap between generated and reference reports. Recognizing their inability to capture clinical accuracy, we secondly employ the GREEN metric~\cite{ostmeier2024green}, a state-of-the-art framework that uses an LLM judge (GPT-4o-mini) (refer to Tab.~\ref{tab:green_metric_prompt} for the corresponding prompt) to estimate the factual and clinical correctness of radiology reports (Fig.~\ref{fig:report_generator}c). Finally, to directly measure the Mammo-GRG's ability to identify key mammographic findings, we perform two complementary evaluations. First, on the BU and UPMC datasets -- where ground-truth radiology reports are available -- we compare the findings from the generated and reference reports (\eg mass, calcification \etc). Using GPT-4o-mini, we extract structured labels for mass, calcification, and asymmetry from both reports and compute Recall to quantify how well the generated reports recover true findings (Fig.~\ref{fig:report_generator}d). This report-vs-report setup measures whether the Mammo-GRG reproduces clinically relevant information, described by the radiologists. Second, on datasets with image-label annotations such as VinDr (OOD) and EMBED (ID), we evaluate the pathological grounding of the generated report. Similar to the previous setup, we parse the generated report using GPT-4o-mini into structured labels for mass and calcification. Finally, we compare these parsed labels directly against the ground truth findings to compute the Recall metric. This report-vs-label evaluation measures the Mammo-GRG’s ability to generate descriptions that align with actual imaging findings. We benchmark Mammo-GRG against MedGemma-27B and LLaVA-Med. As these baselines accept only a single image, we generate a report for each of the four views independently and concatenate the results. To enable a more direct comparison of the underlying visual representations, we also create variants of our multi-view architecture that substitute the Mammo-CLIP vision encoder with the encoders from MedGemma-27B and LLaVA-Med, keeping all other components constant. We denote these two baselines as MedGemma (Finetuned) and LLaVA-Med (Finetuned).

Mammo-GRG, leveraging the Mammo-CLIP (multi-institution) vision encoder, outperforms all the baselines across all evaluation settings. Figures \ref{fig:report_generator}e–f summarize results on the BU and UPMC datasets, showing consistent performance gains in BLEU-1, ROUGE-L, and GREEN scores over all baseline models. The improvement is most evident in clinical correctness measured by the GREEN metric. On the BU dataset, Mammo-GRG achieves a GREEN score of 0.38 $\pm$ 0.18, representing a 58\% improvement over MedGemma (Finetuned) (0.24 $\pm$ 0.12) and a more than fivefold gain over LLaVA-Med (Finetuned)(0.06 $\pm$ 0.02). Similarly, on the UPMC dataset, Mammo-GRG achieves a GREEN score of 0.42 $\pm$ 0.35, yielding a 62\% improvement over MedGemma (Finetuned) (0.26 $\pm$ 0.21) and a sixfold increase relative to LLaVA-Med (Finetuned) (0.06 $\pm$ 0.14). This improvement in clinical accuracy extends to the Mammo-G
RG’s ability to recover key mammographic findings from generated reports when compared to the original ground-truth reports (Fig.~\ref{fig:report_generator}g and Fig.~\ref{fig:app_birads_metric}). On the BU dataset, Mammo-GRG achieves higher recall than fine-tuned MedGemma by 45\%, 18\%, and 52\% for masses (0.61 \vs 0.42), calcifications (0.70 \vs 0.59), and asymmetry (0.47 \vs 0.31), respectively ($P \textless 0.001$ for all comparisons). On the UPMC dataset, Mammo-GRG delivers consistent gains over fine-tuned MedGemma, achieving 43\%, 26\%, and 45\% higher recall for masses (0.57 \vs 0.40), calcifications (0.78 \vs 0.62), and asymmetry (0.42 \vs 0.29), respectively ($P \textless 0.001$ for all of them). Refer to Fig.~\ref{fig:app_report_accuracy} for analogous comparisons using the accuracy metric. To further assess clinical generalization, we evaluate the generated reports against ground-truth mammographic labels rather than reference reports (Fig.~\ref{fig:report_generator}h). On the OOD VinDr dataset, Mammo-GRG achieves a 103\% and 95\% higher recall for suspicious calcifications (0.59 \vs 0.29) and masses (0.43 \vs 0.22), respectively ($P = 0.004$ for both), compared to the base MedGemma model. On the in-distribution EMBED dataset, Mammo-GRG maintains strong predictive alignment, achieving a 68\% and 114\% gain for calcifications (0.45 \vs 0.27, $P \textless 0.001$) and masses (0.30 \vs 0.14), respectively ($P \textless 0.001$ for both of them), relative to fine-tuned MedGemma. Mammo-GRG derives factual grounding directly from Mammo-CLIP’s zero-shot grounding to align generated text with visual evidence without requiring labels or retraining. This approach is inexpensive to deploy yet delivers strong cross-domain generalization. When annotated data are available, Mammo-GRG integrates supervised adaptation using a linear probe or full fine-tuning to further enhance factual consistency. Fine-tuning increases precision but demands substantial computational and annotation cost. Refer to Fig.~\ref{fig:app_mammo_grg_ft} and ~\ref{fig:app_ablation_mammo_GRG_LLM_quantitative} for a detailed comparison of performance of these grounding strategies. Refer to Tab.~\ref{tab:app_ablation_mammo_GRG_llms} for a comparison of the effects of different LLM choices (Llama-3.1-8B \vs Vicuna-13B \vs Mistral-7B) on Mammo-GRG. 
Together, these findings establish Mammo-GRG as the first clinically grounded, multi-view mammography report generation model. Mammo-GRG delivers consistent diagnostic accuracy across lexical, clinical, and pathological axes, setting a new benchmark for trustworthy AI in breast-imaging practice.

% Our multi-view report generator, powered by the Mammo-CLIP vision encoder, consistently outperforms all baseline models across both standard and clinical-focused metrics. The advantage is particularly clear when we assess for clinical correctness using the GREEN metric. On the UPMC dataset, our model achieves a GREEN score of 0.43, representing a 153\% improvement over the original MedGemma (0.17).  
% Fig.~\ref{fig:report_generator}g evaluates findings from report
% This superior clinical fidelity translates to substantially improved recall for critical mammographic findings on the UPMC dataset; compared to the original MedGemma, our model improves recall by 66\% for calcifications (0.78 \vs 0.47), 104\% for masses (0.51 \vs 0.25), and over 200\% for asymmetry (0.51 \vs 0.17). To isolate the contribution of the vision encoder, we compare our model to a variant using the MedGemma encoder within our multi-view framework. Even in this direct comparison, Mammo-CLIP’s specialized features provide a clear advantage, boosting the calcification recall from 0.57 to 0.78 on the UPMC dataset. 

% This robust generalization is particularly evident on the out-of-distribution (OOD) VinDr dataset for findings critical to cancer diagnosis. Here, our model achieves a recall of 0.59 for suspicious calcifications and 0.43 for masses—improvements of 103\% and 54\%, respectively, over the original MedGemma baseline. (Fig.~\ref{fig:report_generator}h)

% Also Fig.~\ref{fig:report_generator}e and Fig.~\ref{fig:report_generator}f tells BLEU-1 and ROUGE-L and GREEN for BU and UPMC respectively. 



